Entropy, concentration, and learning: a statistical mechanics primer

Artificial intelligence models trained through loss minimization have demonstrated significant success, grounded in principles from fields like information theory and statistical physics. This work explores these established connections through the lens of statistical mechanics, starting from first-principles sample concentration behaviors that underpin AI and machine learning. Our development of statistical mechanics for modeling highlights the key role of exponential families, and quantities of statistics, physics, and information theory.

==> ICLR_sufficient_dimension_reduction.tex <==
\section{Sufficient dimensionality reduction}

We seek to learn a good representation of data $X$, which is nearly sufficient to predict $X$ using a black-box decoder model $f$. 
So we are looking to 


\section{Formulation}


\section{History}

The 



\section{Chain of thought}

Start with a black-box model $f (x) \in X$. 
We want to evaluate that model with some test distribution $D \in X$. 

We can condition on different contexts $c \in X$, which do influence the output. 
So there is a way of making some $f_{\mid c} (x)$, with the property that $f_{\mid c}$ takes into account $c$, and "follows this instruction," i.e. is constrained by $c$. 
On the parts of the data indicated by $c$ (addressed by $c$), $f_{\mid c}$ should "take into account" what c says, through a constraint $C (c)$. 
The constraint should be some average over data; 
in fact the constraint can just bound predictions on new data, generated synthetically somehow following $C (c)$

We can make $c_0$ zero-shot, and this causes $f_{\mid c_0} (x)$. 
Based on the mistakes, we can make $c_1$; and so on, iteratively modifying the constraints and shrinking the constraint set. 

\begin{itemize}
\item 
How to choose a new constraint -- greedy like in adaboost?
\item 
How to generate a constraint set $C (c)$?
\item 

\end{itemize}


==> SMD_conditioning_examples.tex <==
\section{Advanced properties of exponential families}

\subsection{The log-likelihood, Cramér-Rao, and stability at equilibrium}

Again remember our constraints $\mathcal{A}$. 
For any $P_{\lambda}$ in the exponential family, we know that: 
$$ \log P_{\lambda} (x) = - A (\lambda) + \sum_{i=1}^{d} \lambda_{i} f_{i} (x) $$

Therefore,  
\begin{align*}
\frac{\partial \log P_{\lambda} (x)}{\partial \lambda_i } 
&= f_{i} (x) - \mathbb{E}_{x \sim P_{\lambda}} \left[ f_i(x) \right]
\end{align*}

Now this is a probability distribution, so taking $\frac{\partial}{\partial \alpha_{i}}$ of both sides: 
\begin{align*}
\mathbb{E} [P_{\lambda} (x)] - 1 = 0 \implies \mathbb{E} \left[ \frac{\partial P_{\lambda} (x)}{\partial \alpha_{i}} \right] = 0
\end{align*}

Similarly, we have the moment constraint $\alpha_{i} = \mathbb{E}_{x \sim P_{\lambda}} \left[ f_{i} (x) \right]$, so 
\begin{align*}
\alpha_{i} = \mathbb{E}_{x \sim P_{\lambda}} \left[ f_{i} (x) \right] \implies 
1 = \mathbb{E}_{} \left[ \frac{\partial P_{\lambda} (x)}{\partial \alpha_{i}} f_{i} (x) \right]
\end{align*}

Therefore, 
\begin{align*}
1 &= \mathbb{E}_{} \left[ \frac{\partial P_{\lambda} (x)}{\partial \alpha_{i}} f_{i} (x) \right] 
= \mathbb{E}_{} \left[ \frac{\partial P_{\lambda} (x)}{\partial \alpha_{i}} ( f_{i} (x) - \alpha_{i} ) \right] \\
&= \mathbb{E}_{} \left[ \frac{\partial [ \log P_{\lambda} (x) ]}{\partial \alpha_{i}} P_{\lambda} (x) ( f_{i} (x) - \alpha_{i} ) \right] 
= \mathbb{E}_{x \sim P_{\lambda}} \left[ \frac{\partial [ \log P_{\lambda} (x) ]}{\partial \alpha_{i}} ( f_{i} (x) - \alpha_{i} ) \right]
\end{align*}

By Cauchy-Schwarz between vectors $\frac{\partial [ \log P_{\lambda} ]}{\partial \alpha_{i}} (x)$ and $f_{i} (x) - \alpha_{i}$, 
\begin{align}
\label{eq:crbound}
1 &\leq \sqrt{ \mathbb{E}_{x \sim P_{\lambda}} \left[ \left( \frac{\partial [ \log P_{\lambda} (x) ]}{\partial \alpha_{i}} \right)^2 \right] \mathbb{E}_{x \sim P_{\lambda}} \left[ ( f_{i} (x) - \alpha_{i} )^2 \right] }
\end{align}



\subsection{Cramér-Rao equalities and exponential families}

The bound \Cref{eq:crbound} is an equality \cite{wijsman1973attainment, joshi1976attainment, van2013detection} when the two vectors are parallel, or proportional, so that for some constant $C_{i}$, 
\begin{align*}
C_{i} (f_{i} (x) - \alpha_{i}) = \frac{\partial [ \log P_{\lambda} (x) ]}{\partial \alpha_{i}}
\end{align*}

When does this happen? 
Multiplying both sides by $(f_{j} (x) - \alpha_{j})$ and taking the expectation with respect to $P_{\lambda}$, 
\begin{align*}
C_{i} \mathbb{E}_{x \sim P_{\lambda}} \left[ (f_{i} (x) - \alpha_{i}) (f_{j} (x) - \alpha_{j}) \right]
&= \mathbb{E}_{x \sim P_{\lambda}} \left[ \frac{\partial [ \log P_{\lambda} (x) ]}{\partial \alpha_{i}} (f_{j} (x) - \alpha_{j}) \right] \\
&= \mathbb{E}_{} \left[ \frac{\partial P_{\lambda} (x)}{\partial \alpha_{i}} (f_{j} (x) - \alpha_{j}) \right] \\
&= \mathbb{E}_{} \left[ \frac{\partial P_{\lambda} (x)}{\partial \alpha_{i}} f_{j} (x) \right] \\
\end{align*}

We have just shown that $\mathbb{E}_{} \left[ \frac{\partial P_{\lambda} (x)}{\partial \alpha_{i}} f_{j} (x) \right] = \textbf{1} (i = j)$, i.e. $1$ if $i=j$ and $0$ otherwise. 
Therefore, $C_{i} = \left( \mathbb{E}_{x \sim P_{\lambda}} \left[ (f_{i} (x) - \alpha_{i})^{2} \right] \right)^{-1}$. 






% Under this distribution, we can calculate the distribution $P_E$ over energy levels. 
% If $M (h)$ is the set of microstates with energy $E (\cdot) = h$, i.e. $M (h) := \left\{ x \in \mathcal{X} : E (x) = h \right\}$, 
% then 
% \begin{align*}
% P_E (h) = \int_{M (h)} P_{\mathcal{A}}^{*} (x) d x 
% \end{align*}

% Then all microstates with this particular energy have the same probability under the max-ent distribution 
% And there are how many of them? It's just one halfspace constraint corresponding to the max-ent parameters; the entropy of the resulting max-ent distribution (i.e., under this one halfspace constraint)
% \begin{align*}
% \text{Pr} \left( \hat{P}_n \in \mathcal{A} \right)
% \end{align*}

% The number of microstates at a particular energy is simply the ratio between the probability at the energy and the probability of an individual microstate with that energy. 




\section{Conditional learning problems}


In learning situations with any supervision, we are tasked with learning a conditional distribution of some variables $y$, **given** some covariates $x$. 

\subsection{Conditional and marginal distributions}

Suppose we condition on some subset of the feature functions $f_{\mathcal{B}} (x) = (f_i (x))_{i \in \mathcal{B}}$.  
Then the conditional distribution of the data is also an exponential family, with the same log-partition function, as shown below. 

Recall that the distribution of the data is of the form

\begin{align*}
Q (x \mid \lambda) = h (x) \exp \left( \lambda^\top f (x) - A (\lambda) \right)
\end{align*}

\begin{align*}
Q_{\lambda} (f_{ \mathcal{B}} (x)) = \exp \left( \lambda_{ \mathcal{B}}^\top f_{\mathcal{B}} (x) - A (\lambda) \right) g_1 \left( f_{ \mathcal{B}} (x), \lambda_{ \mathcal{\tilde{B}}} \right)
\end{align*}


\begin{align*}
Q_{\lambda} \left( f_{ \mathcal{\tilde{B}}} (x) \mid f_{ \mathcal{B}} (x) \right) = \exp \left( \lambda_{ \mathcal{\tilde{B}}}^\top f_{\mathcal{\tilde{B}}} (x) - A (\lambda_{ \mathcal{\tilde{B}}}) \right) g_2 \left( f_{ \mathcal{B}} (x), \lambda_{ \mathcal{\tilde{B}}} \right)
\end{align*}


\subsection{Deviance residuals}

If there are, these will show up as directions along which the data has low entropy, right?
And therefore those can iteratively be learned basis functions?

https://www.cs.columbia.edu/~blei/fogm/2018F/materials/Efron2018.pdf

The deviance between the data (or any distribution in $\mathcal{A}$) and an exponential family is exactly this divergence $\text{D} (P \mid\mid P_{\lambda})$ \cite{efron2022exponential}. 
It can be decomposed over the data's featurization, and analysis of deviance methods are popular ways to isolate structure in the data.


\subsection{How conditional exponential families manifest}

- \cite{BF15, BF15b, BF16} papers as being about conditional exponential families. Typical setup with discrete given $x$, prediction of $y \mid x$. 





\section{Notes}

Generalized forces can be plotted for each data point, with respect to each of its coordinates (and/or with respect to others). 





\section{Examples}

Most of the distributions encountered in statistics are exponential families. 
The received wisdom in statistics is that exponential families need to have exponential tails, and that fat-tailed distributions like the $t$ and Cauchy are not exponential families. 
This is not true, as we show next. 


\subsection{Univariate distributions}

The prototypical commonly known exponential-tail distributions fall into the exponential family, as is widely known. 

- Exponential
- Gaussian
- Gamma


Less well-known examples include many fatter-tailed distributions, including the prototypical Cauchy, Student's t, and Pareto distributions: \texttt{https://www.sciencedirect.com/science/article/abs/pii/S0304407608002200}


- Cauchy
- Student's t distribution: \cite{preda1982student}
- Pareto: \cite{guiasu1990classification}
- Generalized gamma: \cite{preda1984informational}
- Generalized Pareto: \cite{singh1995parameter} 
- Weibull: This applies max-ent constraints of $X^{k}$ and $\ln X$.
- GEV: \cite{singh1998entropy} file:///Users/akshay/Downloads/(Water%20Science%20and%20Technology%20Library%2030)%20Vijay%20P.%20Singh%20(auth.)%20-%20Entropy-Based%20Parameter%20Estimation%20in%20Hydrology-Springer%20Netherlands%20(1998).pdf



\subsection{Multivariate distributions}

- Gaussian
- Multivariate Liouville: \cite{bhattacharya2006maximum}


\begin{align*}
 \textbf{Distribution} \quad& \textbf{Parameters}  \quad& \textbf{Sufficient statistics} \quad& \\ 
 \hline \hline
 \text{Exponential} \quad& \lambda \in \mathbb{R} \quad& \{ x, x^2 \} \quad& \\ 
 \hline \hline
 \text{$t$ (Student)} \quad& \nu \in \mathbb{N} \quad& \left\{ \ln \left( 1 + \frac{x^2}{\nu} \right) \right\} \quad& \\ 
 \hline \hline
 \text{Pareto} \quad& m \in \mathbb{N} \quad& \{ x, \ln (x) \} \quad&  \\
 \text{Generalized extreme value} \quad& cell9 \quad& \{ x, \ln (x) \} \quad&  \\
 \hline \hline
 \text{Multivariate Gaussian} \quad& m \in \mathbb{N} \quad& \{ x, \ln (x) \} \quad&  \\
 \text{Multivariate Liouville} \quad& cell9 \quad& \{ x, \ln (x) \} \quad&  \\
\end{align*}



\subsection{Conditional distributions}

In a standard supervised learning setting, we condition on some high-dimensional data $X$ and look to predict $\text{Pr} (y \mid X)$, the conditional distribution of the labels. 
Many standard prediction models his conditional distribution also corresponds to models conditional-entropy 



Now the covariates are partitioned into an $x, y$. 
We have samples from the joint distribution, and many more samples from the distribution over just $x$, marginalized over $y$. 
And we wish to model the conditional distribution $P (y \mid x)$. 

In this context, the max-entropy method incorporates the conditional distribution's statistics, often the only stably inferrable quantity from little data. 
Statistical mechanics 

Maximizing conditional entropy is also equivalent to minimizing the mutual information between $X$ and $Y$ under moment and marginal constraints on the joint distribution \cite{globerson2003sufficient}:

\begin{align*}
\min I (X, Y)
\end{align*}

See also eq. 5 in \cite{globerson2003sufficient} and the discussion around it. https://www.jmlr.org/papers/volume3/globerson03a/globerson03a.pdf

Logistic regression: code it up and benchmark against standard implementations. 
Experimental setting in \cite{mao2023cross} https://proceedings.mlr.press/v202/mao23b/mao23b.pdf - we can clearly use ResNet 50/34/18 as the feature extractor, and then logistic regression on top.

Then there is https://github.com/UCSC-REAL/cifar-10-100n

And other settings in SAM \cite{foret2020sharpness}. 



\subsubsection{GLMs and exponential families}

Note how the noise model inevitably leads to GLM

This actually provides a different perspective on the statistics.

Network / SAE


\subsubsection{Application: classifier errors}

What is the behavior of classifier errors given some observed joint frequencies? ME can solve this nicely. And also get fluctuations around the mean statistic, i.e. what would be confidence sets containing empirical frequencies?



\subsubsection{Chow-Liu tree learning and structure learning}

https://www.cs.cmu.edu/~aarti/Class/10701/slides/Lecture19.pdf

==> SMD_expfamex_short.tex <==
\section{Exponential families and their properties}
\label{sec:expfamex}

Everything we have described so far leads to the key role of the distribution $P_{\mathcal{A}}^{*}$ over $\mathcal{X}$. 
It is the target distribution according to all the perspectives of learning mentioned earlier: log-loss minimization with exponential family $\mathcal{Q}$, robust Bayes under observations $\mathcal{A}$, and probability calculation of 

\Cref{sec:boltzmanncalc} has shown that the basic quantities of information theory, like (cross) entropy, emerge from first principles when calculating probabilities of fluctuations in sampling from a discrete distribution. 
The calculation, performed first by Boltzmann, shows that high-entropy configurations are exponentially more likely than other configurations. 

This happens to an overwhelming degree in the macroscopically sized samples of atoms we observe in everyday life: our observations are almost deterministic, even of highly disordered systems like gaseous and liquid matter. 

From a modeling perspective, exponential family distributions are extremely useful, as we have described in \Cref{sec:seclearning}. 
It's worth describing them a little more comprehensively, with a view to setting up the stat-mech interpretation of these learning problems, and unlock some more of their power for the prediction problems fundamental to machine learning. 


\subsection{The information projection revisited}

See e.g. \cite{follmer2011stochastic}, Thm. 3.24 for the following

**Theorem**: Given a multivariate random variable $X \in \mathbb{R}^d$, and a constraint vector $S$, the maximum entropy distribution $Q^*$ that satisfies the constraint $\mathbb{E}_{Q^*} [X] = S$ is given by the exponential tilting of the original distribution $P$, 
for some $\lambda^* \in \mathbb{R}^d$ such that $\mathbb{E}_{Q^*} [X] = S$:
$$ Q^* := \arg \min_{Q : \mathbb{E}_{Q} [X] = S} \; D (Q \mid \mid P)  \;\;\iff\;\;  Q^* \propto P \exp \left( \lambda^{* \top} X \right) \text{\;\;with\;\;} \mathbb{E}_{Q^*} [X] = S $$
Therefore, the minimized KL divergence is 
$$ \min_{Q : \mathbb{E}_{Q} [X] = S} \; D (Q \mid \mid P) = \lambda^{* \top} S $$



Let's $\text{D} (Q \mid\mid P)$




Then the maximum entropy distribution is the distribution that maximizes the entropy subject to the constraints that the expected value of each feature function is fixed: 

$$
\begin{aligned}
\max_{P} & \quad \text{H}(P) := \mathbb{E}_{x \sim P} [- \log P(x) ] \\
\text{s.t.} & \quad \mathbb{E} [ f_i(x) ] = \alpha_i \quad \text{for all } i = 1, \dots, d.
\end{aligned}
$$

The distribution that solves this is given by 
$$ P_{\mathcal{A}}^{*} (x) := P_{\lambda^*} (x) \propto \exp \left( \sum_{i=1}^{d} \lambda_i^* f_i(x) \right) $$

where $\left\{ \lambda_i^* \right\}_{i=1}^{d}$ are Lagrange multipliers that enforce the constraints. 

The exponential family associated to features $f (x) \in \mathbb{R}^{d}$ is given by 
\begin{align*}
\mathcal{Q}
:= 
\left\{ P (x \mid \lambda) \in \Delta(\mathcal{X}): \exists \lambda \in \mathbb{R}^{d} : \;
P (x \mid \lambda) \propto h (x) \exp \left( \sum_{i=1}^{d} \lambda_{i} f_{i} (x) \right) \right\}
\end{align*}
where the log-partition function 
$ \displaystyle
A (\lambda) := \log \mathbb{E} \left[ \exp \left( \sum_{i=1}^{d} \lambda_i f_i(x) \right) \right]
$. 


Here I collect the known properties of exponential families. 
I'm aiming to be as complete as possible, though evidently all properties can in principle be derived from the definition of the exponential family so far. 





\subsection{Sufficient statistics and factorizations}

A major motivating principle behind exponential families is that they are exactly the distributions with sufficient statistics whose dimension does not grow with the amount of data, i.e. a parametric model. 
This is known as the Pitman-Koopman-Darmois theorem on sufficient statistics \cite{fisher1922mathematical, koopman1936distributions, Darmois1935, pitman1936sufficient}. 
We won't prove this result for now, as it's rigorously proven already; it's important, but as it's not very practically applicable given our existing explorations into exponential families, we will omit it here. 

A similarly central place is taken by the factorization theorem for pdf's characterizing sufficient statistics, also studied in depth around that time \cite{neyman1935suunteorema} and shown to be a very general perspective on sufficiency \cite{halmos1949application}. 
The general idea of the proof is interesting and fundamental
\footnote{Here is a short proof for the discrete case $\mathcal{X} = \{ X_1, \dots, X_n \}$. 
In this case, the factorization theorem says that any statistic $T(X)$ is sufficient if and only if the probability mass function (PMF) of $X$ can be factored as $f_n (X|\theta) = u(X)v(T(X), \theta)$ for some functions $u$ and $v$. 
We prove both directions of the implication in turn. 

First, assume that the PMF of $X$ can be factored as above. Then:
$ \displaystyle P(T = t) = \sum_{x:T(x) = t} P(X = x) = v(t, \theta) \sum_{x:T(x)=t} u(x) $. 
The conditional distribution of $X$ given $T$ is:

$
P(X = x | T = t) = \frac{P(X = x, T = t)}{P(T = t)} = \frac{u(x)}{\sum_{x:T(x)=t} u(x)}
$

Since this expression does not depend on $\theta$, $T(X)$ is a sufficient statistic.

Conversely, if we start by assuming $T(X)$ is sufficient, we can factor 
$
P(X = x | \theta) = P(X = x | T = t)  P(T = t | \theta)
$. 
Let $ u(x) = P(X = x | T = t) $ and $ v(t, \theta) = P(T = t | \theta) $, giving the factorization $ P(X = x | \theta) = u(x)v(T(x), \theta) $. 
This proves the converse direction and the result.}, 
shown to hold for exponential families. 

Exponential families are vital for graph-based inference as well. 
For any graph structure (CRF), any exponential family over it is going to factorize over the cliques in the graph structure, and furthermore the distributions that factorize like this are exactly the ones that obey the Markov property with respect to the graph. 
This is often called the Hammersley-Clifford theorem, or the Gibbs-Markov theorem. 
Though the result is extremely unique and general, its proof is essentially straightforward, and is given in \cite{Pollard04, besag1974spatial}. 

It also means that if we are satisfied with exponential-family conditional distributions on each edge of the graph (we have settled on some edge-wise features), we can as well restrict ourselves to exponential-family joint distributions over the graph. 

Useful practical graphs have sparse connectivity, admitting practically informative factorizations. 
Arbitrary architectures by decoupling the roles of inputs and outputs. 

%see https://originalstatic.aminer.cn/misc/billboard/aml/Hammersley-Clifford%20Theorem.pdf , (http://www.stat.yale.edu/~pollard/Courses/251.spring04/Handouts/Hammersley-Clifford.pdf)




\subsection{Data-generating "robustness"}

Exponential families are remarkably easy to compare to each other.  
For any distributions $P_{\alpha}, P_{\beta}$ from the same exponential family $\mathcal{Q}$, and any distribution $Q$, we have 

\begin{align*}
\text{D} (Q \mid\mid P_{\beta}) - \text{D} (Q \mid\mid P_{\alpha}) 
&= \mathbb{E}_{x \sim Q} \left[ \log \left( P_{\alpha} (x) \right) - \log \left( P_{\beta} (x) \right) \right] \\
&= \mathbb{E}_{x \sim Q} \left[ \left( \sum_{i=1}^{d} \alpha_i f_i(x) - A (\alpha) \right) - \left( \sum_{i=1}^{d} \beta_i f_i(x) - A (\beta) \right) \right] \\
&= \sum_{i=1}^{d} (\alpha_i - \beta_i ) \mathbb{E}_{x \sim Q} \left[ f_i(x) \right] - A (\alpha) + A (\beta) \qquad \qquad (*)
\end{align*}


This key equation $(*)$ has a few important consequences when $Q \in \mathcal{A}$. 
Suppose $Q, P_{\alpha} \in \mathcal{A}$, i.e. the data follow the same moment constraints as one of the distributions. 
Then, 
\begin{align*}
\text{D} (Q \mid\mid P_{\beta}) - \text{D} (Q \mid\mid P_{\alpha}) 
&= \sum_{i=1}^{d} (\alpha_i - \beta_i ) \mathbb{E}_{x \sim Q} \left[ f_i(x) \right] - A (\alpha) + A (\beta) \\
&= \sum_{i=1}^{d} (\alpha_i - \beta_i ) \mathbb{E}_{x \sim P_{\alpha}} \left[ f_i(x) \right] - A (\alpha) + A (\beta) \\
&= \mathbb{E}_{x \sim P_{\alpha}} \left[ \log \left( \frac{P_{\alpha} (x)}{P_{\beta} (x)} \right) \right] 
= \text{D} (P_{\alpha} \mid\mid P_{\beta})
\end{align*}

This is called "robustness" of exponential families \cite{grunwald2007minimum}: 
the relative performance of two coding schemes $P_{\alpha}, P_{\beta}$ is the same when measured by any $Q \in \mathcal{A}$. 
In our situation, it means that if $\hat{P}_{n}$ denotes the observed data distribution and $P_{\mathcal{A}}^{*}$ the max-entropy distribution under the observed features, 
then for any $P_{\lambda} \in \mathcal{Q}$, 
\begin{align*}
\text{D} (\hat{P}_{n} \mid\mid P_{\lambda}) - \text{D} (\hat{P}_{n} \mid\mid P_{\mathcal{A}}^{*}) 
&= \text{D} (P_{\mathcal{A}}^{*} \mid\mid P_{\lambda})
\end{align*}

In other words, the relative performance of any model $P_{\lambda}$ to the best $P_{\mathcal{A}}^{*}$ is the same when measured on any distribution $P \in \mathcal{A}$ that meets observable moment constraints. 
If for instance, $P_{\mathcal{A}}^{*} \in \mathcal{A}$ is used for $P$, . 

\textbf{For measuring the relative loss of two distributions within the family, we can pretend the data follows $P_{\mathcal{A}}^{*}$. }

All this has been true with "performance" being measured by regret. 
Note that for any distributions, 
\begin{align*}
\text{D} (Q \mid\mid P_{\beta}) - \text{D} (Q \mid\mid P_{\alpha})
= 
\text{H} (Q , P_{\beta}) - \text{H} (Q , P_{\alpha})
\end{align*}
so all these statements are true for loss as well. 







\subsection{Approximation and estimation error}

Substituting any two distributions $Q_1, Q_2 \in \mathcal{A}$ into $(*)$ above: 
\begin{align*}
\text{D} (Q_1 \mid \mid P_{\gamma}) - \text{D} (Q_1 \mid \mid P_{\lambda}) &- \text{D} (Q_2 \mid \mid P_{\gamma}) + \text{D} (Q_2 \mid \mid P_{\lambda}) \\
&= \mathbb{E}_{x \sim Q_1} \left[ \log \left( \frac{P_{\lambda} (x)}{P_{\gamma} (x)} \right) \right] 
- \mathbb{E}_{x \sim Q_2} \left[ \log \left( \frac{P_{\lambda} (x)}{P_{\gamma} (x)} \right) \right] \\
&= \sum_{i=1}^{d} (\lambda_i - \gamma_i ) \left( \mathbb{E}_{x \sim Q_1} \left[ f_i(x) \right] - \mathbb{E}_{x \sim Q_2} \left[ f_i(x) \right] \right) 
= 0
\end{align*}

Setting $Q_1 = P_{\gamma} = P_{\mathcal{A}}^{*}$ for any $P_{\mathcal{A}}^{*} \in \mathcal{A} \cap \mathcal{Q}$, we get a very useful result about this max-entropy distribution $P_{\mathcal{A}}^{*}$: it satisfies a Pythagorean theorem for any $P$ meeting the moment constraints ($P \in \mathcal{A}$), and any $P_{\lambda} \in \mathcal{Q}$. 
\begin{align*}
\underbrace{\text{D} (P \mid\mid P_{\lambda}) }_{\text{regret}} = \underbrace{\text{D} (P_{\mathcal{A}}^{*} \mid\mid P_{\lambda})}_{\text{estimation error}} + \underbrace{\text{D} (P \mid\mid P_{\mathcal{A}}^{*})}_{\text{approximation error}}
\end{align*}

This is a decomposition of the relative loss (the regret) into estimation and approximation errors. 

\begin{itemize}
\item
The approximation error is lowered by considering more expressive architectures. 
\item
The estimation error is lowered by considering more data. 
\end{itemize}

This means that if all we know about the data is encapsulated in $\mathcal{A}$, it is a good idea to minimize over the parametric family $\mathcal{Q}$ (under the geometry induced by $\text{D}$). 
There are some specific consequences to the Pythagorean equality above. 



\subsection{Consequences of MLE}

The maximum likelihood estimation problem is solved by minimizing the log loss -- the cross entropy between the data and the model predictions. 
In our notation, we can formulate this as: 
\begin{align*}
\min_{\lambda} \; \text{D} (\hat{P}_{n} \mid\mid P_{\lambda})
\end{align*}
where $\hat{P}_{n}$ is the empirical distribution of the data.

Since the data $\hat{P}_{n} \in \mathcal{A}$ by definition, from above, $\text{D} (\hat{P}_{n} \mid\mid P_{\lambda}) \geq \text{D} (\hat{P}_{n} \mid\mid P_{\mathcal{A}}^{*}) \quad \forall \lambda$. 
The : 
\begin{align*}
\text{D} (\hat{P}_{n} \mid\mid P_{\lambda}) \geq \text{D} (\hat{P}_{n} \mid\mid P_{\mathcal{A}}^{*}) \quad \forall \lambda
\end{align*}




\subsection{Breaking down the approximation error}

For any data meeting the constraints, i.e. $P \in \mathcal{A}$: 
\begin{align*}
\text{H} (P_{\mathcal{A}}^{*}) - \text{H} (P) 
&= \text{D} (P \mid\mid P_{\mathcal{A}}^{*})
\end{align*}

Therefore, the data will be well approximated if they have roughly maximal entropy under the constraints, i.e. there aren't un-included constraints that really influence the problem. 


Tying together these concepts, the max-entropy problem has a variational characterization: $\text{H} (P_{\lambda^{*}}) - \text{H} (P) = \text{D} (P \mid\mid P_{\lambda^{*}})$ for all $P$ matching the moment constraints. 
This extends to any moment constraints, so we equivalently have for any $\lambda$ that 
\begin{align*}
\text{H} (P_{\lambda}) - \text{H} (P) = \text{D} (P \mid\mid P_{\lambda})
\end{align*}
for all $P$ having the same feature moments as $P_{\lambda}$.





\subsection{Evaluating exponential-family models}

Using this in the regret decomposition above, 
\begin{align*}
\underbrace{\text{D} (P \mid\mid P_{\lambda}) }_{\text{regret}} &= \text{D} (P_{\mathcal{A}}^{*} \mid\mid P_{\lambda}) + \text{H} (P_{\mathcal{A}}^{*}) - \text{H} (P) \\
&= \text{H} (P_{\mathcal{A}}^{*} , P_{\lambda}) - \text{H} (P) 
\end{align*}

Adding $\text{H} (P)$ to both sides gives an interesting result: 
\begin{align*}
\forall P \in \mathcal{A} : \qquad \qquad \text{H} (P , P_{\lambda}) &= \text{H} (P_{\mathcal{A}}^{*} , P_{\lambda})
\end{align*}

\textbf{For evaluating the loss using an exponential family, we can pretend the data follows the max-ent distribution. }




\subsection{Using data to approximate the exponential family}

If we flip the roles of $P$ and $P_{\mathcal{A}}^{*}$ in the above question about divergence, we see that 
$$ - \text{D} (P_{\mathcal{A}}^{*} \mid \mid P) \geq \frac{1}{n} \log \text{Pr} ( \hat{P}_{n} \in \mathcal{A} ) $$

So if $\hat{P}_{n}$ is consistent with the observations $\mathcal{A}$ and $\text{Pr} ( \hat{P}_{n} \in \mathcal{A} )$ is high, then $\text{D} (P_{\mathcal{A}}^{*} \mid \mid P)$ is quite low - the data $P$ is a good approximation to samples generated with $P_{\mathcal{A}}^{*}$. 

It won't affect free energy and KL divergence, which are regret-type measures which already pretty much correct for the inherent (Bayes) loss in describing the data. 


% <!-- $$ \text{D} (P_1 \mid\mid Q_1) + \text{D} (P_2 \mid\mid Q_2) - \text{D} (P_1 \mid\mid Q_2) - \text{D} (P_2 \mid\mid Q_1) = \lambda ( \mathbb{E}_{x \sim P_1} [f] - \mathbb{E}_{x \sim P_2} [f] ) $$ -->





\subsection{Miscellaneous properties}

Similarly, for any $\lambda$ used as a prior to define the exponential family, 
the actual data is harder to encode than the max-ent distribution. 
\begin{align*}
\text{D} (P \mid\mid P_{\lambda}) \geq \text{D} (P_{\mathcal{A}}^{*} \mid\mid P_{\lambda}) \quad \forall P \in \mathcal{A}
\end{align*}

The dual of the log-loss minimization problem is the max-entropy problem (see \cite{DPDPL97}, among others). 





\subsection{The log-partition function and Bregman divergences}

A well-known result \cite{chowdhury2023bregman} connects the cumulant-generating function of the features to the log-partition function $A (\lambda)$ of the exponential family.

\begin{align*}
\log \mathbb{E}_{x \sim P_{\lambda}} \left[ \exp \left( \sum_{i=1}^{d} \lambda_i f_i(x) \right) \right] 
&= A (\lambda + \lambda) - A (\lambda) \\
\implies \\
\log \mathbb{E}_{x \sim P_{\lambda}} \left[ \exp \left( \sum_{i=1}^{d} \lambda_i \left( f_i(x) - \mathbb{E}_{x \sim P_{\lambda}} [f_i (x)] \right) \right) \right] 
&= A (\lambda + \lambda) - A (\lambda) - \lambda^\top \nabla A (\lambda)
\end{align*}



\subsection{Higher moments and fluctuations}

In \Cref{sec:fluctuationsgaussian}, we discussed how to view the probability distribution over less-visited states. 
Now that we have a formula for the distribution, it is time to discuss the special relationship between higher moments and the Fisher information. 

Fisher information: https://www.stat.purdue.edu/~dasgupta/expfamily.pdf . Further calculations from https://cba.mit.edu/events/03.11.ASE/docs/Wainwright.1.pdf

We can look at fluctuations by looking at the distribution over microstates $\mathcal{X}$, 
which we already know we can treat as $P_{\mathcal{A}}^{*}$. 
Under this distribution, we can calculate the distribution $P_E$ over energy levels. 
If $M (h)$ is the set of microstates with energy $E (\cdot) = h$, i.e. $M (h) := \left\{ x \in \mathcal{X} : E (x) = h \right\}$, 
then 
\begin{align*}
P_E (h) = \int_{M (h)} P_{\mathcal{A}}^{*} (x) d x 
\end{align*}

Then all microstates with this particular energy have the same probability under the max-ent distribution 
And there are how many of them? It's just one halfspace constraint corresponding to the max-ent parameters; the entropy of the resulting max-ent distribution (i.e., under this one halfspace constraint)
\begin{align*}
\text{Pr} \left( \hat{P}_n \in \mathcal{A} \right)
\end{align*}

The number of microstates at a particular energy is simply the ratio between the probability at the energy and the probability of an individual microstate with that energy. 
This is often approximated by assuming the probability distribution near the optimum to be roughly Gaussian: 
\begin{align*}
dfkj
\end{align*}




\section{Statistical mechanics: energy and loss minimization}

We arrive at our main task -- laying out the properties of this learning task using a rigorous statistical mechanics viewpoint, drawing a web of connections between statistical physics, information theory, and learning. 


\subsection{Internal energy}

Let's now define the \textbf{internal energy} that the EF associates with any microstate $x$ as 
$$ U_i^{\lambda} (x) := - \lambda_i f_i (x)$$ 
This is the energy of the system in state $x$ associated with the $i$-th feature, which adds to make the total energy $ U^{\lambda} (x) := \sum_{i=1}^{d} U_i^{\lambda} (x) $, 
so that $P_{\lambda} (x) \propto \exp \left( - \sum_{i=1}^{d} U_i^{\lambda} (x) \right) = \exp \left( - U^{\lambda} (x) \right)$. 
Taken over distributions, we have 
$$ U^{\lambda} (P) := - \sum_{i=1}^{d} \lambda_i \mathbb{E}_{x \sim P} [f_i (x)] = \mathbb{E}_{x \sim P} \left[ \sum_{i=1}^{d} U_i^{\lambda} (x) \right] $$ 

At equilibrium (when the expected moments match the empirical moments), the internal energy is $- \sum_{i=1}^{d} \lambda_i \alpha_i$ where $\alpha_i$ are the supplied constraints. 



\subsection{Free energy}

The \textbf{free energy} is simply the max-ent Lagrangian:

$$ F^{\lambda} (P) := U^{\lambda} (P) - \text{H}(P) = - \sum_i \lambda_i \mathbb{E}_{x \sim P} [f_i (x)] - \text{H}(P) $$

so that $F^{\lambda} (P_{\lambda}) = - A (\lambda)$. And we have for any $P$ matching the moment constraints that 

$$ F^{\lambda} (P) - F^{\lambda} (P_{\lambda}) = \text{D} (P \mid\mid P_{\lambda}) $$

This is the dual interpretation (minimum free energy at fixed temperature) to the usual primal variational characterization (maximum entropy at fixed energy). 



The log-partition function is:
\begin{align*}
A ( \lambda ) &:= \min_{Q \in \Delta(\mathcal{X})} \;\max_{P \in \Delta(\mathcal{X})} \left[ \text{H} (P, Q) - U^{\lambda} (P) \right] \\
&= \max_{P \in \Delta(\mathcal{X})} \left[ \text{H} (P) + \sum_{i=1}^{d} \lambda_{i} \mathbb{E}_{x \sim P} [ f_{i} (x) ] \right]
= \log \mathbb{E} \left[ \exp \left( \sum_{i=1}^{d} \lambda_i f_i(x) \right) \right]
\end{align*}



\subsection{Entropy}

The entropy of the exponential family $P_{\lambda}$ is 
\begin{align*}
\text{H} (P_{\lambda}) 
&:= U^{\lambda} (P_{\lambda}) - F^{\lambda} (P_{\lambda}) \\
&= \sum_{i=1}^{d} - \lambda_i \mathbb{E}_{x \sim P_{\lambda}} \left[ f_i(x) \right] + \log \mathbb{E} \left[ \exp \left( \sum_{i=1}^{d} \lambda_i f_i(x) \right) \right]
= - \sum_{i=1}^{d} \lambda_i \alpha_i + A (\lambda)
\end{align*}



\subsection{Loss and internal energy}

For any distribution $P$ whatsoever, and any parameters $\lambda$, the loss $\mathbb{E}_{x \sim P} \left[ - \log (P_{\lambda} (x)) \right] = \text{H} (P, P_{\lambda})$ is: 
$$ 
\text{H} (P, P_{\lambda})
=
A (\lambda) - \sum_i \lambda_i \mathbb{E}_{x \sim P} [f_i (x)]
= U^{\lambda} (P) - F^{\lambda} (P_{\lambda})
\qquad \qquad
(*)
$$

In other words, for any $\lambda$: 
$$\text{H} (x, P_{\lambda}) = - \sum_{i=1}^{d} \lambda_{i} f_{i} (x) + A (\lambda) = U^{\lambda} (x) - F^{\lambda} (P_{\lambda}) $$



If the loss is low, $U^{\lambda} (x) \approx F^{\lambda} (P_{\lambda})$, which is highly negative; so the energy is generally negative over the data! 

Therefore, for any two arbitrary distributions $P, Q$: 
\begin{align*}
\text{H} (P, P_{\lambda}) - \text{H} (Q, P_{\lambda})
= U^{\lambda} (P) - U^{\lambda} (Q)
\end{align*}


This shows that gaps in internal energy of distributions directly reflect gaps in $P_{\lambda}$'s prediction performance on them. 

Internal energy of data would be high when $P_{\lambda}$ is a poor code for the data, low otherwise. 
It's the excess loss over that if the data were distributed according to the model $P_{\lambda}$.

If the data are relatively well-described by the model, the regret/free energy will be low. 
If the data are also pretty low-entropy, the internal energy will be low.


\subsection{Regret and free energy}

Subtracting $H(P)$ from both sides of the equation $(*)$, we get as above that 
\begin{align*}
\text{D} \left( P \mid \mid P_{\lambda} \right) = F^{\lambda} (P) - F^{\lambda} (P_{\lambda})
\end{align*}

which is a very good variational characterization of the free energy. 
For us, it takes special significance as a tight bound on the (zero-centered) loss -- the *regret*. 

In most cases for $P$, expectation values would be easiest to compute, so $U(P)$ is certainly more amenable to computation than $H (P)$.





\subsection{The log-likelihood, Cramer-Rao, and stability at equilibrium}

$$ \log P_{\lambda} (x) = - A (\lambda) + \sum_{i=1}^{d} \lambda_{i} f_{i} (x) $$

First note that: 
\begin{align*}
\frac{\partial \log P_{\lambda} (x)}{\partial \lambda_i } 
&= \frac{1}{P_{\lambda} (x)} \frac{\partial P_{\lambda} (x)}{\partial \lambda_i } 
= f_{i} (x) - \mathbb{E}_{x \sim P_{\lambda}} \left[ f_i(x) \right]
\end{align*}

Now this is a probability distribution, so: 
\begin{align*}
\mathbb{E} [P_{\lambda} (x)] - 1 = 0 \implies \mathbb{E} \left[ \frac{\partial P_{\lambda} (x)}{\partial \alpha_{i}} \right] = 0
\end{align*}

and therefore, 
\begin{align*}
\alpha_{i} = \mathbb{E}_{x \sim P_{\lambda}} \left[ f_{i} (x) \right] &\implies \\
1 &= \mathbb{E}_{} \left[ \frac{\partial P_{\lambda} (x)}{\partial \alpha_{i}} f_{i} (x) \right] \\
&= \mathbb{E}_{} \left[ \frac{\partial P_{\lambda} (x)}{\partial \alpha_{i}} ( f_{i} (x) - \alpha_{i} ) \right] \\
&= \mathbb{E}_{} \left[ \frac{\partial [ \log P_{\lambda} (x) ]}{\partial \alpha_{i}} P_{\lambda} (x) ( f_{i} (x) - \alpha_{i} ) \right] \\
&\leq \sqrt{ \mathbb{E}_{x \sim P_{\lambda}} \left[ \left( \frac{\partial [ \log P_{\lambda} (x) ]}{\partial \alpha_{i}} \right)^2 \right] \mathbb{E}_{x \sim P_{\lambda}} \left[ ( f_{i} (x) - \alpha_{i} )^2 \right] }
\end{align*}

Carry on from [@tikochinsky1984alternative], stability analysis. 

\begin{align*}
d \alpha_{i} = d \mathbb{E}_{x \sim P_{\lambda}} \left[ f_{i} (x) \right]
 = \mathbb{E} \left[ P_{\lambda} (x) d f_{i} (x) + d P_{\lambda} (x) f_{i} (x) \right]
\end{align*}

From above, if $\frac{\partial f_{i} (x)}{\partial \alpha_i } = 0$, 
\begin{align*}
\frac{\partial \log P_{\lambda} (x)}{\partial \alpha_i } 
&= \sum_{j=1}^{d} \left[ \frac{\partial \lambda_{j}}{\partial \alpha_i } ( f_{j} (x) - \alpha_j ) \right]
\end{align*}


A general version of this calculation leads to the Cramer-Rao lower bound. 
See "informal derivation" for more. 









\subsection{Mean-field approximation: Bogoliubov's inequality}

The information projection we are discussing has another convenient property for learning, when looking to approximate it with another "\textit{variational}" model distribution. 

For any variational $P_{\psi}$ with $U^{\psi} (P_{\psi}) = U^{\psi} (P_{\lambda})$, we have 
\begin{align*}
0 &\leq \text{D} (P_{\lambda} \mid\mid P_{\psi}) \\ 
&= \sum_{i=1}^{d} (\lambda_i - \psi_i ) \mathbb{E}_{x \sim P_{\lambda} } \left[ f_i(x) \right] - A (\lambda) + A (\psi) \\
&= \sum_{i=1}^{d} \left( \lambda_i \mathbb{E}_{x \sim P_{\lambda} } \left[ f_i(x) \right] - \psi_i \mathbb{E}_{x \sim P_{\psi} } \left[ f_i(x) \right] \right) - A (\lambda) + A (\psi )\\
&= U^{\psi} (P_{\psi}) - U^{\lambda} (P_{\lambda}) + F^{\lambda} (P_{\lambda}) - F^{\psi} (P_{\psi}) \\
&= \text{H} (P_{\psi}) - \text{H} (P_{\lambda}) = F^{\lambda} (P_{\lambda}) - F^{\psi} (P_{\psi})
\end{align*}





\section{Discussion}



\subsection{Statistical mechanics interpretations}

Intensive vs extensive variables are replaced by observables vs parameters. 
Neither the heat nor the entropy are pointwise observable quantities - they are both properties of the system (dataset) as a whole, and heat is additionally a property of the change between datasets. 

This is the Helmholtz free energy; the Gibbs and other free energies are just derived by first privileging the volume constraint (fix pressure), then the energy (fix temp). 


In applications of statistical mechanics to physics, the energy constraint is treated specially \cite{landau2013statistical}. 
In general the energy is a special privileged constraint, with $f_1$ being the Hamiltonian. 

Let's specialize to this case, considering one constraint -- the **privileged** constraint -- $f_1$. 
The maximum-entropy distribution is then given by $P_{\mathcal{A}}^{*} (x) \propto \exp \left( \lambda_1 f_1(x) \right)$.

\begin{itemize}
\item 
The Lagrange multiplier $\lambda_1$ is the inverse **temperature** $T_1 := 1/\lambda_1$ associated with $f_1$. 

\item 
The internal energy associated with $f_1$ is $U_1 = \mathbb{E}_{x \sim P_{\lambda}} [f_1 (x)] = \mathbb{E}_{x \sim P_{\lambda}} [f_1 (x)] = - \frac{\partial }{\partial \lambda_1} [A (\lambda)]$ where $A$ is the log-partition function. 

\item 
The free energy associated with $f_1$ is the Lagrangian: $F_1 (P) := \mathbb{E}_{x \sim p} [f_1 (x)] - \frac{1}{\lambda_1} \text{H} (P) $. For $P_{\lambda}$, it is $ = - \frac{1}{\lambda_1} [A (lambda)]$. 
For any $p$ matching moment constraints, $F_1 (P) - F_1 (P_{\lambda}) = \text{D} (p \mid\mid P_{\lambda})$.
\end{itemize}



\subsection{Interpretation}

\begin{itemize}
\item 
\textbf{Constant pressure/temperature} processes are those where the $\lambda$ doesn't change. 

\item
\textbf{Constant-volume} processes are those where there is no mechanical work done. Here, we hold $W$ constant, i.e. $\Delta_{i} (x) = 0$ on average. 

\item
\textbf{Heat} is the change in energy that is not due to work, but associated with entropy of the configuration. https://physics.stackexchange.com/questions/315381/specific-heat-in-isothermal-and-adiabatic-process-for-gas

\item
\textbf{Constant-energy} processes are those where the internal energy (performance) is held constant, so work and heat exactly offset each other.

\item
\textbf{Intensive} quantities are the model parameters ($\lambda$ values), and **extensive** quantities are those that depend on the data $x$. The Euler equation applies to all our quantities that are 0-homogeneous here.

\item
\textbf{Quasi-static processes} are those where the infinitesimal entropy change and heat change are proportional. In our case, $\mathbb{E}_{x \sim P_{\lambda}} [f_{i} (x)] - \alpha_{i} = 0$. 

\item
\textbf{Adiabatic processes} are those where the heat change is zero, i.e. $\delta Q_i^{\lambda} = 0$ for all $i$. 
I.e. when $\mathbb{E}_{x \sim P_{\lambda}} \left[ \Delta_{i} (x) \right] = \Delta_{i}^{\alpha}$ for all $i$. 

\item
\textbf{Reversible processes} are those where the entropy is conserved, and the process is quasi-static ($\mathbb{E}_{x \sim P_{\lambda}} [f_{i} (x)] = \alpha_{i}$). 

\item
\textbf{Irreversible processes} are those where entropy is produced within the system; consequently, in order to maintain constant entropy within the system, energy must be simultaneously removed from the system as heat. 

\item
\textbf{Equilibrium} is running a process until $\lambda$ is a max-ent solution. Once $\alpha_i$ is changed, the system will evolve to a new max-ent solution represented by new parameters $\lambda$. 
\end{itemize}

- A notion of **specific heat** of a dataset is: 
% (http://john.maloney.org/cruelest_equation.htm) [@landau2013statistical] https://www2.ph.ed.ac.uk/~mevans/sp/sp3.pdf

$$ T_{i} \frac{\partial \text{H} (P_{\lambda})}{\partial T_{i}} = - \lambda_{i} \frac{\partial \text{H} (P_{\lambda})}{\partial \lambda_i} = - \lambda_{i} \left( \mathbb{E}_{x \sim P_{\lambda}} [f_{i} (x)] - \alpha_{i} \right) $$

- A notion of "temperature" of a dataset is just $\frac{\partial U}{\partial \text{H}}$ when holding $W$ constant (see [@pathria2021statistical])
- **Efficiency** is the ratio of work done to heat absorbed. We can define this as the ratio of the change in entropy to the change in internal energy.


The inverse of the temperature is the cost of buying energy from the rest of the world. The lower the temperature, the more strongly the
energy is pushed downward. Entropy is the currency being paid. For each unit of energy $\delta E$ bought, we pay $\delta E/T = \delta E (dS/dE) = \delta S$ in reduced entropy of the outside world. Inverse temperature is the cost in entropy to buy a unit of energy (More correctly, one pays in negative entropy; one must accept entropy $\delta E/T$ when buying energy $\delta E$ from the heat bath.)



- Instead of a microstate calculation motivating max (cross-?)entropy , we have a minimax loss problem motivating it

- Instead of extensive observables constraining the entropy, we have expectations over feature functions constraining it


Entropy is concave in internal energy, and so $\frac{\partial^2 \text{H} (P_{\lambda}) }{\partial E^2} = - \lambda_{i}^{2} \frac{\partial (1/\lambda_i) }{\partial E}$, and so inverse temperature $\lambda_i$ decreases with increasing energy, as we would expect. 


\subsection{Le Chatelier's principle}

https://chemistry.stackexchange.com/questions/104165/can-le-chateliers-principle-be-derived

OR result of concavity of entropy in terms of observables.

\subsection{Generalized forces}

Since early modern statistical mechanics [@khinchin1949mathematical], the concept of generalized forces has been present. Generalized forces represent sensitivity of internal/free energy to other parameters. 

\begin{itemize}
\item 
Generalized forces are the dual variables of the constraints (https://arxiv.org/pdf/1903.02121) - the Lagrange parameters. 

\item 
Generalized forces can be plotted for each data point, with respect to each of its coordinates (and/or with respect to others).

\item 
The book [@kardar2007statistical] has a good exposition

\item 
Generalized displacements (extensive variables, features, observed variables) are involved in Le Chatelier's principle https://arxiv.org/pdf/1609.02308
\end{itemize}





\subsection{A philosophical shift}

This entails a philosophical shift in the way we think about data and modeling. 

The modeling here, though it does ultimately involve $d$ parameters, does not make parametric assumptions about the data. 
Once features are chosen for a dataset, there is always a best $\lambda^*$ which satisfies the feature constraints at their observed data-derived values. 

This is a very different way of thinking about data than the traditional parametric approach, where we assume a fixed number of parameters and try to estimate them.
It privileges a particular distribution - the maximum-entropy distribution - over all others, as it is by far the most likely to have generated the data. 
We can effectively treat the data as if it came from this distribution, and calculate deviations accordingly. 
In other words, our choice to featurize and observe the data in a particular way is the only assumption we make about the data -- this **determines** the distribution of the data within strict bounds, exactly as our observations of atoms are constrained to certain known bulk properties. 

Entropy is the worst-case loss in general, and when there is underlying "physics" to motivate a uniform prior, we can derive the fundamental link between entropy and multiplicity that appears on Boltzmann's tombstone. 
Our analogous "physics" is the empirical sampling process that leads to the training set; the i.i.d. assumption with the test distribution. 
But from a loss minimization perspective, cross-entropy is actually the more fundamental quantity being optimized. 




\subsection{The many faces of (cross) entropy}

Cross entropy is a measure of the divergence between two probability distributions. 
Entropy itself has many interpretations, including from an information-theoretic point of view. \cite{cover1994processes}

The axiomatic basis of entropy and cross-entropy is now a widely studied topic. 
Shannon \cite{shannon1948} had a development of information theory and Khinchin \cite{khinchin1949mathematical} of statistical mechanics -- these "Shannon-Khinchin axioms" were foundational in future work. 
Other important treatments followed, notably a set of natural axioms justifying cross-entropy as a loss function for prediction and inference \cite{shore1980axiomatic}. 

- Relative entropy justified in \cite{van1981maximum} as the limit of some conditional distributions
- More axioms in \cite{skilling1988axioms} and \cite{csiszar1991least}





\subsection{Connections to thermal physics and information theory}

We are following the mathematical development of statistical mechanics, developed in physics to study the behavior of observables in systems of many particles. 
In physics, these ideas are fully mature, but require certain laws of physics to be valid, most notably the uniform distribution over phase space (Liouville's theorem). 

In information theory, the same ideas are used to study the behavior of observables in systems of many bits. 
The spirit of the statistical mechanics applications is significantly generalized to apply to arbitrary distributions over data, and arbitrary sample sizes. 

Studying these ideas from a prediction perspective, we can unlock some more generality and power in the formalism, and bring some of the accumulated understanding of statistical mechanics to bear on the problem of prediction in machine learning.



\subsubsection{Thermodynamics of computation}

See \cite{bennett1982thermodynamics}, \cite{zurek1989algorithmic}, \cite{szilard1964decrease}, 

There is a thermodynamic cost to computation.



\subsection{Information theory preliminaries}

Information theory describes distributions over some set of possible outcomes $\mathcal{X}$. 
The basic definition we work from is the cross entropy of a distribution $Q$ with respect to another distribution $P$: 
$$ \text{H} (P, Q) := \mathbb{E}_{x \sim P} \left[ - \log (Q(x)) \right] $$

This gives rise to the notions of entropy (the minimum cross entropy) and KL divergence (the regret to the minimum cross entropy):

\begin{align*}
\text{H} (P) &:= \text{H} (P, P) = \min_{Q} \text{H} (P, Q) = \mathbb{E}_{x \sim P} \left[ - \log (P(x)) \right]
\\
\text{D} (P \mid \mid Q) &:= \text{H} (P, Q) - \text{H} (P) = \mathbb{E}_{x \sim P} \left[ \log \left( \frac{P(x)}{Q(x)} \right) \right]
\end{align*}





\subsection{Misc}

See \cite{lesne2014shannon} https://www.lptmc.jussieu.fr/user/lesne/MSCS-entropy.pdf - Sec 8.3 on concentration of measure of entropy, going back to \cite{einstein1910theorie}. 


It turns out that cross-entropy is the only loss with the dual probability-based perspective we've discussed in \Cref{sec:subequivlearning} \cite{tikochinsky1984alternative}. 



==> SMD_generalized_thermodynamics.tex <==
\section{The equations of generalized statistical mechanics}


Ref [@jiao2015justification], [@dawid2007geometry], [@GD04], [@BF16], [@dawid2014theory]

I've set up the formalism of statistical mechanics, using maximum-entropy methods as a bridge between decision theory and thermodynamics. 
But there's still one fundamental assumption: the log loss. 
While extremely useful and probably the most common loss function in machine learning, it's not the only one. 
We would like to generalize the ideas in the statistical mechanics framework to other prediction situations.
This makes the math work out, which seems like a magical coincidence; 
how much of this is due to the general principles of statistical mechanics?

Generalizing this requires generalizing the statistical mechanical tools we have developed. 


Entropy, which is so fundamental in the thermodynamic calculation of probabilities of microstates, has a different role in the decision-theoretic setting. 
In the decision-theoretic setting, the entropy is a measure of uncertainty, ultimately stemming from the use of cross-entropy as a loss function. 

\section{Alternative loss functions}

- Proper scores and Bregman divergences: [@mccarthy1956measures] and [@jose2008scoring]. Also [@dawid2014theory] shows 
construct a proper scoring rule from any loss; see also Raf's work e.g. 

- The paper [@ovcharov2018proper] shows a 
of theory behind proper losses.

- $https://healy.econ.ohio-state.edu/papers/Chambers_Healy_Lambert-Duality.pdf$ gives a main result that's provable with the minimax theorem, and extends [@GD04], stretching the notion of proper losses to include an arbitrary utility function of the $L (\delta_{x}, Q)$ loss vector (instead of just a linear one). 

- See also [@cerreia2011uncertainty] file:///Users/akshay/Downloads/JET201120120928154931.PDF

- Define max-ent distributions, Pythagorean theorem, etc. from [@GD04]. For those, derive statmech. 


\subsection{Loss function}

THe loss function $\text{H} (P, Q)$ is a measure of the divergence between target distribution $P$ and predicted distribution $Q$. 
We assume it is linear in $P$, depending on the function $\text{H} (x, Q)$ for each $x$ in the support of $P$. 

Further properties of $\text{H} (x, Q)$ determine the properties of the loss function: 

- We require $\text{H} (x, Q)$ to be proper, such that $\arg \min_{Q \in \Delta (\mathcal{X})} \text{H} (x, Q) = \delta_{x}$, then $\text{H} (P, Q)$ is a proper loss function.
- If $\text{H} (x, Q)$ is local, i.e. depends only on $Q(x)$, and if it's a monotonic function of $Q$, its expression can be inverted to explicitly write $Q$.


\subsection{Derived losses and energy}

\begin{align*}
\text{H} (P) := \text{H} (P, P) = \min_{Q} \text{H} (P, Q)
\qquad 
\text{D} (P \mid \mid Q) := \text{H} (P, Q) - \text{H} (P)
\end{align*}

The **internal energy** is
$$ U^{\lambda} (P) := - \sum_{i=1}^{d} \lambda_i \mathbb{E}_{x \sim P} [f_i (x)] = \mathbb{E}_{x \sim P} \left[ \sum_{i=1}^{d} U_i^{\lambda} (x) \right] $$
where $U_i^{\lambda} (x) := - \lambda_i f_i (x)$ is the energy of the system in state $x$ associated with the $i$-th feature, which adds to make the total energy $ U^{\lambda} (x) = \sum_{i=1}^{d} U_i^{\lambda} (x) $. 

At equilibrium (when the expected moments match the empirical moments), the internal energy is $- \sum_{i=1}^{d} \lambda_i \alpha_i$. 

The **free energy** is simply the Lagrangian

$$ F^{\lambda} (P) := U^{\lambda} (P) - \text{H}(P) = - \sum_i \lambda_i \mathbb{E}_{x \sim P} [f_i (x)] - \text{H}(P) $$



\subsection{Generalized exponential family distributions}

The **generalized exponential family (GEF)** $P_{\lambda}$ is: 

\begin{align*}
P_{\lambda} := \arg \min_{Q \in \Delta(\mathcal{X})} \;\max_{P \in \Delta(\mathcal{X})} \left[ \text{H} (P, Q) - U^{\lambda} (P) \right]
\end{align*}

The value of this game is the log-partition function:

\begin{align*}
A ( \lambda ) := \min_{Q \in \Delta(\mathcal{X})} \;\max_{P \in \Delta(\mathcal{X})} \left[ \text{H} (P, Q) - U^{\lambda} (P) \right] 
= \max_{P \in \Delta(\mathcal{X})} \left[ \text{H} (P) - U^{\lambda} (P) \right]
= \max_{P \in \Delta(\mathcal{X})} \left[ - F^{\lambda} (P) \right]
\end{align*}

It can be proven that the unique optimal strategies for both players are the GEF distribution $P_{\lambda}$. 
This has deep consequences. 

- $F^{\lambda} (P_{\lambda}) = - A (\lambda)$

- $\text{H} (x, P_{\lambda}) = U^{\lambda} (x) + A ( \lambda )$ (equalizer rule proof in [@GD04]; local proper scoring rules make this the definition of $P_{\lambda} (x)$). 

This means that for any distribution $P$, 
$$\text{H} (P, P_{\lambda}) - U^{\lambda} (P) = \text{H} (P_{\lambda}) - U^{\lambda} (P_{\lambda}) = A (\lambda)$$


\subsection{Energy and loss}

Rearranging gives a formula for the internal energy:

\begin{align*}
U^{\lambda} (P) = \text{H} (P, P_{\lambda}) - A (\lambda)
\end{align*}

Internal energy of data would be high when $p^{\lambda}$ is a poor code for the data, low otherwise. 
It's the excess loss over that if the data were distributed according to the model $p^{\lambda}$.
If the data are relatively well-described by the model, the regret/free energy will be low. 
If the data are also pretty low-entropy, the internal energy will be low.

And we have for any $P$ matching the moment constraints that 

\begin{align*}
\text{D} (P \mid\mid P_{\lambda}) &\stackrel{(\mathfrak{P})}{=} \text{H} (P_{\lambda}) - \text{H} (P) \\
&\stackrel{(\mathfrak{D})}{=} F^{\lambda} (P) - F^{\lambda} (P_{\lambda})
\end{align*}

Here $(\mathfrak{P})$ is referred to as the primal variational characterization (maximum entropy at fixed energy) and $(\mathfrak{D})$ is the dual interpretation (minimum free energy at fixed temperature). 

Therefore, the data will be well approximated if they have roughly maximal entropy under the constraints, i.e. there aren't un-included constraints that really influence the problem. 

And if this is not true, there will be constraint(s) along which the data have low entropy, and these can be added to the model to improve the fit. 
This follows Jaynes' philosophy on reasoning, but we don't need to adopt any such philosophy - we're just doing loss minimization. 


The details are determined by a couple of simple equations. 

From [@grunwald2004game] eq (6) **DIFFERENT ONE!**, we have the following:
$$
\max_{P \in \Gamma }\; \text{H} (P, P_{\lambda^{*}}) 
= \text{H} (P_{\lambda^{*}}) 
\leq \min_{q \in \Delta(\mathcal{X})} \;\max_{p \in \Gamma }\; \text{H} (P, Q) 
$$



\section{The laws of thermodynamics}

Recall Khinchin's comment from [@khinchin1949mathematical] about the laws of thermodynamics

> The science of thermodynamics is based essentially on its two fundamental laws...the entire system of thermodynamic theory can be developed logically as a consequence of the two laws.

We do exactly this. 


\subsection{The fundamental thermodynamic relation}

The fundamental thermodynamic relation concerns the differential of the internal energy. 
Recall the fundamental relation above:

\begin{align*}
U^{\lambda} (P_{\lambda}) = F^{\lambda} (P_{\lambda}) + \text{H} (P_{\lambda})
\end{align*}

Now we differentiate with respect to an auxiliary "time" variable $t$, which all the quantities are allowed to vary with. 
This gives the following relations. 



\subsection{First law}

First, we set up a lemma.

Lemma.

Suppose $G (\lambda, P) := \text{H} (P) + \sum_{i=1}^{d} \lambda_{i} \mathbb{E}_{x \sim P} [ f_{i} (x) ]$. 
Then $\max_{P} G (\lambda, P) = A (\lambda)$, with the unique maximizer $P_{\lambda}$. 
This implies that $\max_{\sigma} \left[ G (\sigma, P_{\lambda}) - A (\sigma) \right] = G (\lambda, P_{\lambda}) - A (\lambda) = 0$. 
By the stationary conditions at this optimum, 

\begin{align*}
\frac{\partial A (\sigma)}{\partial \sigma_{i}} 
&= \left[ \frac{\partial G (\sigma, P)}{\partial \sigma_{i}} \right]_{P = P_{\lambda}} \\
&= \mathbb{E}_{x \sim P_{\lambda}} [ f_{i} (x) ] + \sigma_{i} \mathbb{E}_{x \sim P_{\lambda}} \left[ \frac{\partial f_{i} (x)}{\partial \sigma_{i}} \right]
\end{align*}



(This is a version of Danskin's theorem, e.g. [@danskin1966theory], [@madry2018towards].)

The total differential of the free energy is 

\begin{align*}
d A (\lambda)
&= \sum_{i=1}^{d} \left[ \frac{\partial A (\lambda)}{\partial \lambda_{i}} \right]_{P = P_{\lambda}} d \lambda_{i} 
= \sum_{i=1}^{d} \left[ \mathbb{E}_{x \sim P_{\lambda}} [ f_{i} (x) ] d \lambda_{i} + \lambda_{i} \mathbb{E}_{x \sim P_{\lambda}} \left[ d f_{i} (x) \right] \right] \\
&= \mathbb{E}_{x \sim P_{\lambda}} \left[ \sum_{i=1}^{d} \left( f_{i} (x) d \lambda_{i} + \lambda_{i} d f_{i} (x) \right) \right]
= - \mathbb{E}_{x \sim P_{\lambda}} \left[ d U^{\lambda} (x) \right]
\end{align*}



From the above discussion, we can break down the free energy change into heat and work terms, resulting in an analogue to the first law of thermodynamics. 

\begin{align*}
d U^{\lambda} (P_{\lambda})
= d \text{H} (P_{\lambda}) + d [F^{\lambda} (P_{\lambda}) ]
= d \text{H} (P_{\lambda}) + \mathbb{E}_{x \sim P_{\lambda}} \left[ d U^{\lambda} (x) \right]
\end{align*}

So the entropy difference term $d \text{H} (P_{\lambda})$ is the difference $d U^{\lambda} (P_{\lambda}) - \mathbb{E}_{x \sim P_{\lambda}} \left[ d U^{\lambda} (x) \right]$. 



\subsection{Second law}

\begin{align*}
d \text{H} (P_{\lambda})
&= d U^{\lambda} (P_{\lambda}) + d A (\lambda)
= - \sum_{i=1}^{d} \left( d \lambda_{i} \alpha_{i} + \lambda_{i} d \alpha_{i} \right) - \mathbb{E}_{x \sim P_{\lambda}} \left[ \sum_{i=1}^{d} d U_i^{\lambda} (x) \right] \\
&= \sum_{i=1}^{d} \left[ \lambda_{i} \left( \underbrace{\mathbb{E}_{x \sim P_{\lambda}} \left[ d f_{i} (x) \right] - d \alpha_{i}}_{\delta Q_i^{\lambda} } \right) + \left( \mathbb{E}_{x \sim P_{\lambda}} [ f_{i} (x) ] - \alpha_{i} \right) d \lambda_{i} \right]
\end{align*}

<!-- 
It is convenient to differentiate with respect to an auxiliary variable $t$ representing time. 

\begin{align*}
\frac{d \text{H} (P_{\lambda})}{d t} 
&= \frac{d U^{\lambda} (P_{\lambda})}{d t} + \frac{d A (\lambda)}{d t} 
= - \sum_{i=1}^{d} \left( \frac{d \lambda_{i}}{d t} \alpha_{i} + \lambda_{i} \frac{d \alpha_{i}}{d t} \right) - \mathbb{E}_{x \sim P_{\lambda}} \left[ \sum_{i=1}^{d} \frac{\partial U_i^{\lambda} (x)}{\partial t} \right] \\
&= \sum_{i=1}^{d} \left[ \lambda_{i} \left( \underbrace{\mathbb{E}_{x \sim P_{\lambda}} \left[ \frac{d f_{i} (x)}{d t} \right] - \frac{d \alpha_{i}}{d t}}_{\delta Q_i^{\lambda}/\delta t} \right) + \left( \mathbb{E}_{x \sim P_{\lambda}} [ f_{i} (x) ] - \alpha_{i} \right) \frac{d \lambda_{i}}{d t} \right]
\end{align*} -->

We have shown that heat governs change in entropy for a given $\lambda$ at equilibrium (i.e. for a quasi-static process, if $[\partial \lambda] = 0$ so that $\lambda$ is held fixed): 
$$ d \text{H} (P_{\lambda}) = \sum_{i=1}^{d} \lambda_{i} [\delta Q_i^{\lambda}] $$

In general away from equilibrium, we have 

\begin{align*}
d \text{H} (P_{\lambda}) 
= \sum_{i=1}^{d} \left( [d \lambda_{i}] \left( \mathbb{E}_{x \sim P_{\lambda}} [f_{i} (x)] - \alpha_{i} \right) + \lambda_{i} [\delta Q_i^{\lambda}] \right) 
\end{align*}

and so a notion of temperature for each coordinate $i$ in a quasi-static process is $T_{i} = 1/\lambda_{i}$.



\subsection{Differential in loss (local energy)}

\begin{align*}
d \text{H} (x, P_{\lambda})
&= d U^{\lambda} (x) + d A (\lambda) \\
&= d U^{\lambda} (x) - \mathbb{E}_{x \sim P_{\lambda}} \left[ d U^{\lambda} (x) \right]
= - \sum_{i=1}^{d} \left( d \lambda_{i} \alpha_{i} + \lambda_{i} d \alpha_{i} \right) - \mathbb{E}_{x \sim P_{\lambda}} \left[ d U^{\lambda} (x) \right] \\
&= \sum_{i=1}^{d} \left[ \lambda_{i} \left( \underbrace{\mathbb{E}_{x \sim P_{\lambda}} \left[ d f_{i} (x) \right] - d \alpha_{i}}_{\delta Q_i^{\lambda} } \right) + \left( \mathbb{E}_{x \sim P_{\lambda}} [ f_{i} (x) ] - \alpha_{i} \right) d \lambda_{i} \right]
\end{align*}


==> SMD_history.tex <==
How can statistical mechanics be introduced to the uninitiated? 
For one thing, it is the subject of one of the great textbook introductions [@goodstein2014states]:

> Ludwig Boltzmann, who spent much of his life studying statistical mechanics, died in 1906, by his own hand. Paul Ehrenfest, carrying on the work, died similarly in 1933. Now it is our turn to study statistical mechanics. Perhaps it will be wise to approach the subject cautiously...



\section{Why write this?}

The AI changing the world today is largely based on a set of powerful statistical concepts and tools. 
The basic principles involve modeling with loss minimization, which has enjoyed incredible success as a central framework for performing all types of learning. 

The way ahead inevitably involves statistical mechanics, which is the field that studies the properties of matter from its constituent atoms. 
Though it was originally developed for these physics-centric reasons, early pioneers like Gibbs (\cite{gibbs1902elementary}) realized that the math behind it applied to any system of "particles," like a dataset of samples. 

In AI, we must sometimes observe what we can from datasets that are much smaller than physical systems -- instead of moles of constituents, we may have thousands or fewer data points to learn patterns from. 
So it is useful to re-develop and extend some stat-mechanical logic from first principles. 

Emergent ideas like heat and temperature, associated with our physical intuitions, can be linked precisely to the learning and statistical properties of distributions over a dataset. 

In the 1800s, the fields of physics and chemistry were developing quickly from experimental discoveries. 
Bulk properties of matter were measurable to high precision, and scientists searched for the underlying principles that could explain these properties. 
The concept of entropy was developed in this context, and has since emerged as a key idea in the sciences.



\subsection{A brief tour of the entropy concept}

The history of entropy has an unfortunate theme: 
the concept keeps showing its importance in different fields, 
but the degree of complete agreement and unity between all the faces of entropy is not always appreciated. 
We briefly overview some of these facets of entropy. 


\subsubsection{Entropy in statistical physics}

The beginning of the modern concept was probably in the early 1800s, for physics reasons. 
Its understanding dates back to this period, 
when scientists were discovering that thermal heat is a form of energy. 
The practical experimentation that discovered this led to unprecendented development of devices like steam engines. 
Carnot thought about the engineering problems around these during the 1820s, and in 1824 linked engine efficiency to reversibility of physical processes \cite{carnot1978reflexions}. 
The dominant tenor of entropy research that followed focused on the second law of thermodynamics -- the tendency of entropy to increase \cite{clausius1867mechanical} -- and its implications \cite{thomson1851absolute, thomson1857}. 
Boltzmann 

The last of the early giants of the field was Gibbs \cite{gibbs1902elementary}. 
He expressed exponential families in an essentially modern and accurate form, presaging probability theory and information theory in doing so. 
The deterministic appearance of everyday observations was explained by their having such a huge number ($\sim 10^{23}$) of individual constituents. 

Over the early decades of the 20th century, probability theory developed as a discipline, formalizing many of these calculations further. 




\subsubsection{Entropy in information theory}

It was not until WWII and the postwar era that the discipline of information theory formed and grew. 
Shannon \cite{shannon1948} did groundbreaking work justifying entropy axiomatically according to certain intuitive properties of any information measure. 
The field of information theory was then built around this universal notion of information and uncertainty, applying to any possible source. 

Many towering figures contributed to building capabilities around universal compression and storage, which underpin the modern world, making computers possible.  
From our perspective, Kullback and Csiszár are especially important - they recur again and again. 
- Jaynes


So statistical mechanics originated concepts to deal with the behavior of large collections of particles observed in bulk. 
These concepts are probabilistic, so it is very appropriate to examine them 
Information theory originated concepts to deal with the behavior of data and uncertainty, and ultimately links deeply to probability. 
And statistical mechanics and probability are deeply connected as well.


Shannon's original information theory was developed to understand communication, not decision-making; so the focus was on a particular kind of uncertainty. 
But the generalization to decision theory is straightforward, and the connection to statistical mechanics is deep.




\subsubsection{Entropy in loss-driven modeling}

Entropy has a loss minimization perspective as well, which fits perfectly as a complementary view to the others. 
It has been a unifying theme in some key interdisciplinary work from decision theory (\cite{degroot1962uncertainty}, \cite{grunwald2007minimum}, \cite{GD04} and citations therein).




\section{Entropy as an entry point}

The entropy emerges as a natural consequence of some extremely fundamental probability calculations \cite{jaynes1982rationale}. 
Though an elusive concept due to its many uses, it is extremely fundamental in all the situations in which it occurs. 
Since the beginning has related to statistical mechanics. From \cite{tribus1971energy}: 

> My greatest concern was what to call it. I thought of calling it 'information,' but the word was overly used, so I decided to call it 'uncertainty.' When I discussed it with John von Neumann, he had a better idea. Von Neumann told me, 'You should call it entropy, for two reasons. In the first place your uncertainty function has been used in statistical mechanics under that name, so it already has a name. In the second place, and more important, no one knows what entropy really is, so in a debate you will always have the advantage.'

From an AI perspective, it's useful to think about all this in terms of modeling data, in which case max-entropy inference is a widely-known technique that provides a bridge to statistical mechanics. 
This problem can be recast from a loss minimization perspective, which turns out to be much more general when freed of physics considerations. 
As I discuss, the AI/ML/decision-theoretic perspective on these ideas brings out the full generality of statistical mechanics. 

This does not seem to have been discussed previously in the context of exponential families. 
Instead, the focus of the equilibrium and non-equilibrium statistical mechanics variants has been on a thermodynamic formalism, with physics deeply integrated into the theory. 

I take a different perspective, developing statistical mechanics from information theory and divergence minimization. 
This brings out the connections in their most general form, and has roots in deep connections between information theory and probability. 
So the initial focus is a lean, accessible, and deep collection of results on exponential families using the language of information theory. 

==> SMD_thermodynamics.tex <==
The idea here is to develop a different way of looking at the situation, motivated by machine learning and AI. 
When viewed in this light, powerful and principled tools for understanding the most complex models. 

I'll get into the heart of that effort, quantifying changes in the quantities of interest that we established last time: performance and its associated entropy. 
In an AI context, a system is described by a single dataset and a model that is trained on it. 
Therefore, the thermodynamics of systems directly relate to issues of domain shift, generalization, and robustness. 


\section{The laws of thermodynamics}

Schrödinger \cite{schrodinger1948statistical} and Khinchin \cite{khinchin1949mathematical} both sought processes as he explained probability, and what we now recognize as a 

Statistical thermodynamics (\cite{jaynes1957information}, \cite{jaynes1957information2}). 

Khinchin [@khinchin1949mathematical] makes the point that the laws of thermodynamics can be derived purely from statistical-mechanical considerations. 

> The science of thermodynamics is based essentially on its two fundamental laws; thus, every theory pretending to represent the foundation of thermodynamics must prove that these two fundamental laws can be derived from its basic principles. Once this is done, the entire system of thermodynamic theory can be developed logically as a consequence of the two laws.

We do exactly this by deriving the fundamental thermodynamic relation, concerning how the internal energy varies locally. 

Suppose the observed data and the constraints both change, independently. 
Each observed data point changes by $( \Delta_{1} (x), \dots, \Delta_{d} (x)) $. 
The constraints change by $( \Delta_{1}^{\alpha}, \dots, \Delta_{d}^{\alpha} )$. 

$$ f_{i} (x) \impliedby f_{i} (x) + \Delta_{i} (x) \qquad \alpha_{i} \impliedby \alpha_{i} + \Delta_{i}^{\alpha} $$

How much do the properties of the distribution change?


\subsection{Free energy and work}

\begin{align*}
d [\ln Z (\lambda)] &= \frac{1}{Z (\lambda)} d Z (\lambda) 
= \frac{ \sum_{i=1}^{d} \mathbb{E} \left[ \left( [d \lambda_{i}] f_{i} (x) + \lambda_{i} \Delta_{i} (x) \right) \exp \left( \sum_{i=1}^{d} \lambda_i f_i(x) \right) \right] }{\mathbb{E} \left[ \exp \left( \sum_{i=1}^{d} \lambda_i f_i(x) \right) \right]} \\
&= \sum_{i=1}^{d} \left( [d \lambda_{i}] \mathbb{E}_{x \sim P_{\lambda}} [f_{i} (x)] + \lambda_{i} \mathbb{E}_{x \sim P_{\lambda}} \left[ \Delta_{i} (x) \right] \right) \\
&= - \mathbb{E}_{x \sim P_{\lambda}} \left[ \sum_{i=1}^{d} d U_i^{\lambda} (x) \right]
\end{align*}



\subsection{Entropy and heat}

And we can show that 

\begin{align*}
d \text{H} (P_{\lambda}) 
&= d [\ln Z (\lambda)] - d \left[ \sum_{i=1}^{d} \lambda_{i} \alpha_{i} \right] \\
&= \sum_{i=1}^{d} \left[ \left( [d \lambda_{i}] \mathbb{E}_{x \sim P_{\lambda}} [f_{i} (x)] + \lambda_{i} \mathbb{E}_{x \sim P_{\lambda}} \left[ \Delta_{i} (x) \right] \right) - \left( [d \lambda_{i}] \alpha_{i} + \lambda_{i} \Delta_{i}^{\alpha} \right) \right] \\
&= \sum_{i=1}^{d} \left( [d \lambda_{i}] \left( \mathbb{E}_{x \sim P_{\lambda}} [f_{i} (x)] - \alpha_{i} \right) + \lambda_{i} \left( \mathbb{E}_{x \sim P_{\lambda}} \left[ \Delta_{i} (x) \right] - \Delta_{i}^{\alpha} \right) \right) \\
&= \sum_{i=1}^{d} \lambda_{i} [\delta Q_i^{\lambda}]
\end{align*}

where the ``heat change" associated with a given feature $i$ is 
$$ \delta Q_i^{\lambda} := \mathbb{E}_{x \sim P_{\lambda}} \left[ \Delta_{i} (x) \right] - \Delta_{i}^{\alpha} $$



\subsection{First law}

From the above discussion, we can break down the free energy change into heat and work terms, resulting in an analogue to the first law of thermodynamics. 

Recall that 
$$ U^{\lambda} (P) := - \sum_{i=1}^{d} \lambda_i \mathbb{E}_{x \sim p} [f_i (x)] = \mathbb{E}_{x \sim p} \left[ \sum_{i=1}^{d} U_i^{\lambda} (x) \right] $$

\begin{align*}
d U^{\lambda} (P_{\lambda})
= - d \left[ \sum_{i=1}^{d} \lambda_{i} \alpha_{i} \right] 
% = - \left( [d \lambda_{i}] \alpha_{i} + \lambda_{i} \Delta_{i}^{\alpha} \right) 
= d \text{H} (P_{\lambda})  - d [\ln Z (\lambda) ]
= \sum_{i=1}^{d} \left[ \lambda_{i} [\delta Q_i^{\lambda}] + \mathbb{E}_{x \sim P_{\lambda}} \left[ d U_i^{\lambda} (x) \right] \right]
\end{align*}

So the entropy difference term $d \text{H}$ is the difference $d U^{\lambda} (P_{\lambda}) - \sum_{i=1}^{d} \mathbb{E}_{x \sim P_{\lambda}} \left[ d U_i^{\lambda} (x) \right]$. 

In general, 
$ d U^{\lambda} (P_{\lambda}) = - \sum_{i=1}^{d} \left( [d \lambda_{i}] \alpha_{i} + \lambda_{i} \Delta_{i}^{\alpha} \right) $. 

If $[d \lambda] = 0$ so that $\lambda$ is held fixed, this is 
$
d U^{\lambda} (P_{\lambda}) 
= - \sum_{i=1}^{d} \lambda_{i} \Delta_{i}^{\alpha}
$. 


\subsection{Second law}

State this like in \cite{baez2024entropy}. 
The simplest form is probably applying Jensen to Jarzynski's equality. 

At a basic level, this is saying that deviations towards equilibrium tend to privilege higher-entropy distributions, given some moment constraints. Other distributions will tend to have higher loss (energy). 
More atypical initial conditions will tend to degenerate to more typical ones; entropy will increase. 
Lower-entropy fluctuations will lose out to higher-entropy ones. 
If learning new features which tend to lower entropy, the system will tend to the highest-entropy of those. 

We have shown that heat governs change in entropy for a given $\lambda$ at equilibrium (i.e. for a quasi-static process, if $[\partial \lambda] = 0$ so that $\lambda$ is held fixed): 
$$ d \text{H} (P_{\lambda}) = \sum_{i=1}^{d} \lambda_{i} [\delta Q_i^{\lambda}] $$

In general away from equilibrium, we have 

\begin{align*}
d \text{H} (P_{\lambda}) 
= \sum_{i=1}^{d} \left( [d \lambda_{i}] \left( \mathbb{E}_{x \sim P_{\lambda}} [f_{i} (x)] - \alpha_{i} \right) + \lambda_{i} [\delta Q_i^{\lambda}] \right) 
\end{align*}


and so a notion of temperature for each coordinate $i$ in a quasi-static process is $T_{i} = 1/\lambda_{i}$.


**When is heat change zero?**

The first term of heat change is zero when: 
$\mathbb{E}_{x \sim P_{\lambda}} [f_{i} (x)] = \alpha_{i}$ for all $i$ (quasi-static, constraints are satisfied) 
or when $\partial \lambda_{i} = 0$ for all $i$ (no change in parameters). 

The $\delta Q_i^{\lambda}$ term is zero when:
$\mathbb{E}_{x \sim P_{\lambda}} \left[ \Delta_{i} (x) \right] = \Delta_{i}^{\alpha}$ for all $i$ (no change in constraints beyond what is seen in the data)


\subsubsection{Markov chain}

Markov chains ensure that information is only destroyed. 
Under detailed balance (Ex 8.12 of Sethna), free energy decreases. 
This means (see that discussion) that any entropy change isn't fully affecting things, but it's modified by the heat change from the bath. 

This necessarily means entropy increases under a series of data processing operations. 

More generally, pg. 126 of https://www.pbs.org/wgbh/nova/manyworlds/pdf/dissertation.pdf shows that for any MC, $\text{D} (P_{*} \mid\mid P_{n})$ is decreasing.


\subsubsection{Probabilities, low-entropy initializations, and the anthropic principle}

We also have Sanov theorems ensuring control of deviations from typicality. 
Once we're in an atypical state, w.h.p. we won't return. 

Fluctuation theorems break time symmetry, and apply to antisymmetric features. 
They ensure that fluctuations are unidirectional in time with overwhelming probability.

> So either the dynamics observed are time-asymmetric, or the initial configuration is atypical and low-entropy. 




\subsection{Third law}

Again state this like in \cite{baez2024entropy}.

If the loss function has a minimum or is realizable, we should be fine. 

Note the behavior of $H$ at $\lambda \to \infty$ - see Schrodinger ( [@schrodinger1948statistical], Ch. 3). 


\section{Loss differential}

We know that 

\begin{align*}
\text{H} (x, P_{\lambda}) = \sum_{i=1}^{d} U_{i}^{\lambda} (x) + \ln Z (\lambda) 
= U^{\lambda} (x) + \min_{Q \in \Delta(\mathcal{X})} \;\max_{x \in \mathcal{X}} \left[ \text{H} (x, Q) - U^{\lambda} (x) \right] 
= U^{\lambda} (x) + \min_{Q \in \Delta(\mathcal{X})} \text{H}^{*} (\lambda, Q)
\end{align*}

Taking the differential, 
$$ d \text{H} (x, P_{\lambda}) = d U^{\lambda} (x) - \mathbb{E}_{y \sim P_{\lambda}} \left[ d U^{\lambda} (y) \right] $$



\section{Heat-work cycles}


\subsection{Otto cycle}

There are intermediate states, because $f_{i} (x)$ and $\alpha_{i}$ are both different between two states. 

- State 1: $P_{\lambda}$ with constraints $\alpha_{i} = \mathbb{E}_{x \sim P_{\lambda}} \left[ f_{i} (x) \right]$ and feature functions $f_{i} (x)$. 
- State $A_1$: $P_{\lambda}$ with constraints $\alpha_{i} - \delta Q_i^{\lambda}$ and feature functions $f_{i} (x)$.
- State $A_2$: $P_{\lambda}$ with constraints $\alpha_{i} + \mathbb{E}_{x \sim P_{\lambda}} \left[ \Delta_{i} (x) \right] $ and feature functions $f_{i} (x) + \Delta_{i} (x)$. 
- State 2: $P_{\lambda}$ with constraints $\alpha_{i} + \mathbb{E}_{x \sim P_{\lambda}} \left[ \Delta_{i} (x) \right] - \delta Q_i^{\lambda}$ and feature functions $f_{i} (x) + \Delta_{i} (x)$. 

State 1 and 2 are the initial and final states, and state 3 and 4 are intermediate states. 
Suppose $\lambda$ is fixed. 

- $1 \to A_1$: This is pure heat, because the free energy does not change. 
- $A_1 \to 2$: This is adiabatic, zero heat; therefore zero entropy change. 
- $1 \to A_2$: This is adiabatic, zero heat; therefore zero entropy change. 
- $A_2 \to 2$: This is pure heat, because the free energy does not change. 


The pure heat processes are impossible to know fully without observation and sampling. 

We find $A_2$ achievable. What is $U^{\lambda} (A_2)$?


\subsection{Carnot cycle and learning}

If the efficiency of a learning process is measured by the fraction of useful work, then the Carnot cycle is supreme; this also establishes that isentropic processes, where $\lambda$ is maybe changing, are very important. 

Use of Carnot cycle? We don't like heat as it leads to more entropy. We want to just have lower entropy and also lower energy (better performance). 

The behavior of a Carnot engine or refrigerator is best understood by using a temperature–entropy diagram (T–S diagram), in which the thermodynamic state is specified by a point on a graph with entropy (S) as the horizontal axis and temperature (T) as the vertical axis (Figure 2). For a simple closed system (control mass analysis), any point on the graph represents a particular state of the system. A thermodynamic process is represented by a curve connecting an initial state (A) and a final state (B). The area under the curve is:
s
which is the amount of heat transferred in the process. If the process moves the system to greater entropy, the area under the curve is the amount of heat absorbed by the system in that process; otherwise, it is the amount of heat removed from or leaving the system. For any cyclic process, there is an upper portion of the cycle and a lower portion. In T-S diagrams for a clockwise cycle, the area under the upper portion will be the energy absorbed by the system during the cycle, while the area under the lower portion will be the energy removed from the system during the cycle. The area inside the cycle is then the difference between the two (the absorbed net heat energy), but since the internal energy of the system must have returned to its initial value, this difference must be the amount of work done by the system per cycle. Referring to Figure 1, mathematically, for a reversible process, we may write the amount of work done over a cyclic process as:

Since dU is an exact differential, its integral over any closed loop is zero and it follows that the area inside the loop on a T–S diagram is (a) equal to the total work performed by the system on the surroundings if the loop is traversed in a clockwise direction, and (b) is equal to the total work done on the system by the surroundings as the loop is traversed in a counterclockwise direction.

\subsection{Interpretation}

\begin{itemize}
\item 
\textbf{Constant pressure/temperature} processes are those where the $\lambda$ doesn't change. 

\item
\textbf{Constant-volume} processes are those where there is no mechanical work done. Here, we hold $W$ constant, i.e. $\Delta_{i} (x) = 0$ on average. 

\item
\textbf{Heat} is the change in energy that is not due to work, but associated with entropy of the configuration. https://physics.stackexchange.com/questions/315381/specific-heat-in-isothermal-and-adiabatic-process-for-gas

\item
\textbf{Constant-energy} processes are those where the internal energy (performance) is held constant, so work and heat exactly offset each other.

\item
\textbf{Quasi-static processes} are those where the infinitesimal entropy change and heat change are proportional. In our case, $\mathbb{E}_{x \sim P_{\lambda}} [f_{i} (x)] - \alpha_{i} = 0$. 

\item
\textbf{Adiabatic processes} are those where the heat change is zero, i.e. $\delta Q_i^{\lambda} = 0$ for all $i$. 
I.e. when $\mathbb{E}_{x \sim P_{\lambda}} \left[ \Delta_{i} (x) \right] = \Delta_{i}^{\alpha}$ for all $i$. 

\item
\textbf{Reversible processes} are those where the entropy is conserved, and the process is quasi-static ($\mathbb{E}_{x \sim P_{\lambda}} [f_{i} (x)] = \alpha_{i}$). 

\item
\textbf{Irreversible processes} are those where entropy is produced within the system; consequently, in order to maintain constant entropy within the system, energy must be simultaneously removed from the system as heat. 

\item
\textbf{Equilibrium} is running a process until $\lambda$ is a max-ent solution. Once $\alpha_i$ is changed, the system will evolve to a new max-ent solution represented by new parameters $\lambda$. 
\end{itemize}


- **Constant pressure/temperature** processes are those where the $\lambda$ doesn't change. 
- **Constant-volume** processes are those where there is no mechanical work done. Here, we hold $W$ constant, i.e. $\Delta_{i} (x) = 0$ on average. 
- **Heat** is the change in energy that is not due to work, but associated with entropy of the configuration. https://physics.stackexchange.com/questions/315381/specific-heat-in-isothermal-and-adiabatic-process-for-gas
- **Constant-energy** processes are those where the internal energy (performance) is held constant, so work and heat exactly offset each other.
- **Intensive** quantities are the model parameters ($\lambda$ values), and **extensive** quantities are those that depend on the data $x$. The internal energy $U$ would indeed double if the features were all scaled up. The Euler equation applies to all our quantities that are homogeneous here, so $U$ can be rewritten, etc. https://faculty.uca.edu/saddison/Thermal2003/EulerGibbsDuhem.pdf . Neither the heat nor the entropy are pointwise observable quantities - they are both properties of the system (dataset) as a whole, and heat is additionally a property of the change between datasets. 
- **Quasi-static processes** are those where the infinitesimal entropy change and heat change are proportional. In our case, $\mathbb{E}_{x \sim P_{\lambda}} [f_{i} (x)] - \alpha_{i} = 0$. 
- **Adiabatic processes** are those where the heat change is zero, i.e. $\delta Q_i^{\lambda} = 0$ for all $i$. 
I.e. when $\mathbb{E}_{x \sim P_{\lambda}} \left[ \Delta_{i} (x) \right] = \Delta_{i}^{\alpha}$ for all $i$. 
  - **Reversible processes** are those where the entropy is conserved, and the process is quasi-static ($\mathbb{E}_{x \sim P_{\lambda}} [f_{i} (x)] = \alpha_{i}$). 
  - **Irreversible processes** are those where entropy is produced within the system; consequently, in order to maintain constant entropy within the system, energy must be simultaneously removed from the system as heat. 
- **Equilibrium** is running a process until $\lambda$ is a max-ent solution. Once $\alpha_i$ is changed, the system will evolve to a new max-ent solution represented by new parameters $\lambda$. 

- A notion of **specific heat** of a dataset is: 
% (http://john.maloney.org/cruelest_equation.htm) [@landau2013statistical] https://www2.ph.ed.ac.uk/~mevans/sp/sp3.pdf

$$ T_{i} \frac{\partial \text{H} (P_{\lambda})}{\partial T_{i}} = - \lambda_{i} \frac{\partial \text{H} (P_{\lambda})}{\partial \lambda_i} = - \lambda_{i} \left( \mathbb{E}_{x \sim P_{\lambda}} [f_{i} (x)] - \alpha_{i} \right) $$

- A notion of "temperature" of a dataset is just $\frac{\partial U}{\partial \text{H}}$ when holding $W$ constant (see [@pathria2021statistical])
- **Efficiency** is the ratio of work done to heat absorbed. We can define this as the ratio of the change in entropy to the change in internal energy.
- Equipartition theorem is true of all features which are purely quadratic with minimum at $0$, doesn't matter what the proportionality constant on the quadratic is: https://vallance.chem.ox.ac.uk/pdfs/Equipartition.pdf



The inverse of the temperature is the cost in entropy of buying a unit of energy from the rest of the world. 
The lower the temperature, the more strongly the energy is pushed downward. Entropy is the currency being paid. For each unit of energy $\delta E$ bought, we pay $\delta E/T = \delta E (dS/dE) = \delta S$ in reduced entropy of the outside world; one must accept entropy $\delta E/T$ when buying energy $\delta E$ from the heat bath.) 


- The notion of countercurrent exchange can work with equilibrium, if we are willing to stratify the dataset by performance (log loss).


- Instead of a microstate calculation motivating max (cross-?)entropy , we have a minimax loss problem motivating it

- Instead of extensive observables constraining the entropy, we have expectations over feature functions constraining it


Entropy is concave in internal energy, and so $\frac{\partial^2 \text{H} (P_{\lambda}) }{\partial E^2} = - \lambda_{i}^{2} \frac{\partial (1/\lambda_i) }{\partial E}$, and so inverse temperature $\lambda_i$ decreases with increasing energy, as we would expect. 



\subsection{Le Chatelier's principle}

Le Chatelier's principle \cite{chatelier1884enonce} states that 
https://chemistry.stackexchange.com/questions/104165/can-le-chateliers-principle-be-derived

Result of concavity of entropy in terms of observables \cite{pavelka2019braun}. 
See \cite{landaulifshitz} ch 22 . 
The same principle holds quite generally for constrained convex optimization problems \cite{leblanc1976chatelier}, and its significance has been appreciated in fields like economics \cite{samuelson1960extension}. 



\subsubsection{Generalized forces}

Since early modern statistical mechanics [@khinchin1949mathematical], the concept of generalized forces has been present. Generalized forces represent sensitivity of internal/free energy to other parameters. 

- Generalized forces are the dual variables of the constraints (https://arxiv.org/pdf/1903.02121) - the Lagrange parameters. 

- Generalized forces can be plotted for each data point, with respect to each of its coordinates (and/or with respect to others).

- The book [@kardar2007statistical] has a good exposition

- Generalized displacements (extensive variables, features, observed variables) are involved in Le Chatelier's principle https://arxiv.org/pdf/1609.02308




\subsection{Thermodynamics of computation}

See \cite{bennett1982thermodynamics}, \cite{zurek1989algorithmic}, \cite{szilard1964decrease}, 

There is a thermodynamic cost to computation.


\section{What happens when datasets are mixed?}

The new equilibrium distribution has the temperatures the same across all data.


\section{Fluctuation and Maxwell-Onsager relations}

% See also https://itp.uni-frankfurt.de/~gros/Vorlesungen/TD/5_Thermodynamic_potentials.pdf and 

% https://sites.esm.psu.edu/~vfm5153/TSM/lecture8.html




\subsection{Covariance matrix and Fisher information geometry}

\begin{align*}
\frac{\partial \ln Z (\lambda)}{\partial \lambda_{i}} 
&= \frac{1}{Z} \frac{\partial Z (\lambda)}{\partial \lambda_{i}} 
= \frac{1}{Z} \mathbb{E} \left[ f_i (x) \exp \left( \sum_{i=1}^{d} \lambda_i f_i (x) \right) \right]
= \mathbb{E}_{x \sim P_{\lambda}} \left[ f_i(x) \right]
\end{align*}

and 

$$ \frac{1}{Z} \frac{\partial^2 Z (\lambda)}{\partial \lambda_{i} \partial \lambda_{j}} = \mathbb{E}_{x \sim P_{\lambda}} \left[ f_i (x) f_j (x) \right] $$

Differentiating $\ln Z$ again, 

\begin{align*}
\frac{\partial^2 \ln Z (\lambda)}{\partial \lambda_{i} \partial \lambda_{j}} 
&= \frac{\partial \mathbb{E}_{x \sim P_{\lambda}} \left[ f_i (x) \right]}{\partial \lambda_{j}} 
= \frac{\partial \mathbb{E}_{x \sim P_{\lambda}} \left[ f_j (x) \right]}{\partial \lambda_{i}} 
= \mathbb{E}_{x \sim P_{\lambda}} \left[ f_i (x) f_j (x) \right] - \mathbb{E}_{x \sim P_{\lambda}} \left[ f_i (x) \right] \mathbb{E}_{x \sim P_{\lambda}} \left[ f_j (x) \right] 
= \text{cov}_{x \sim P_{\lambda}} \left[ f_i (x), f_j (x) \right]
\end{align*}

This is the Fisher information, because 

\begin{align*}
\frac{\partial^2 \ln Z (\lambda)}{\partial \lambda_{i} \partial \lambda_{j}} 
&= \text{cov}_{x \sim P_{\lambda}} \left[ f_i (x), f_j (x) \right]
= \mathbb{E}_{x \sim P_{\lambda}} \left[ \left( f_i (x) - \mathbb{E}_{x \sim P_{\lambda}} \left[ f_i (x) \right] \right) \left( f_j (x) - \mathbb{E}_{x \sim P_{\lambda}} \left[ f_j (x) \right] \right) \right] \\
&= \mathbb{E}_{x \sim P_{\lambda}} \left[ \left( \frac{\partial [\ln P_{\lambda} (x)]}{\partial \lambda_{i}} \right) \left( \frac{\partial [\ln P_{\lambda} (x)]}{\partial \lambda_{j}} \right) \right] 
\end{align*}




\subsection{Entropy curvature}

\begin{align*}
\frac{\partial \text{H} (P_{\lambda})}{\partial \alpha_i } 
&= \sum_{j=1}^{d} \left[ \frac{\partial \ln Z (\lambda)}{\partial \lambda_{j}} \frac{\partial \lambda_{j}}{\partial \alpha_i } \right] - \frac{\partial [ \sum_{k=1}^{d} \lambda_{k} \alpha_k ]}{\partial \alpha_i } \\
&= \sum_{j=1}^{d} \left[ \frac{\partial \ln Z (\lambda)}{\partial \lambda_{j}} \frac{\partial \lambda_{j}}{\partial \alpha_i } \right] - \lambda_i - \sum_{k=1}^{d} \left[ \frac{\partial \lambda_{k}}{\partial \alpha_i } \alpha_k \right] 
= - \lambda_i
\end{align*}

This can be used as a defining property of the Lagrange multipliers, like temperature (defined as the exponent of the multiplicity, i.e. $d [\log \Omega (E)] / d E = d H / d E$). 
What's the density of the log-partition over features?

Differentiating this again, 

\begin{align*}
- \frac{\partial^2 \text{H} (P_{\lambda}) }{\partial \alpha_{i} \partial \alpha_{j}} 
&= \frac{\partial \lambda_{j}}{\partial \alpha_{i} } 
= \frac{\partial \lambda_{i}}{\partial \alpha_{j} } 
\end{align*}

The matrices $- \frac{\partial^2 \text{H} (P_{\lambda}) }{\partial \alpha_{i} \partial \alpha_{j}}$ and $\frac{\partial^2 \ln Z (\lambda)}{\partial \lambda_{i} \partial \lambda_{j}}$ are inverses of each other, 
as can be verified by the chain rule. 


\subsection{Other differential relations}

We have relations for the derivatives of the log-partition function with respect to the constraints.

\begin{align*}
\frac{\partial \ln Z (\lambda)}{\partial \alpha_i } 
&= \sum_{j=1}^{d} \left[ \frac{\partial \ln Z (\lambda)}{\partial \lambda_{j}} \frac{\partial \lambda_{j}}{\partial \alpha_i } \right] 
= \sum_{j=1}^{d} \left[ \frac{\partial \lambda_{j}}{\partial \alpha_i } \alpha_j \right]
\end{align*}

and finally for the entropy with respect to the Lagrange multipliers:

\begin{align*}
\frac{\partial \text{H} (P_{\lambda}) }{\partial \lambda_{i} } = \mathbb{E}_{x \sim P_{\lambda}} [f_{i} (x)] - \alpha_{i}
\end{align*}



\subsection{Heat capacity}

From above, we have

\begin{align*}
\frac{\partial^2 \ln Z (\lambda)}{\partial \lambda_{i}^2} 
= \frac{\partial [ \mathbb{E}_{x \sim P_{\lambda}} \left[ f_i(x) \right] ]}{\partial \lambda_i } 
= \mathbb{E}_{x \sim P_{\lambda}} \left[ f_i^2 (x) \right] - \left( \mathbb{E}_{x \sim P_{\lambda}} \left[ f_i (x) \right] \right)^{2}
= \text{var}_{x \sim P_{\lambda}} \left[ f_i (x) \right]
\end{align*}

As in Lifshitz, the heat capacity can be identified with the thermal derivative of the average energy:

\begin{align*}
\frac{\partial [ \mathbb{E}_{x \sim P_{\lambda}} \left[ f_i(x) \right] ]}{\ partial T_i } 
= - \lambda_i^2 \frac{\partial [ \mathbb{E}_{x \sim P_{\lambda}} \left[ f_i(x) \right] ]}{\partial \lambda_i } 
= - \lambda_i^2 \text{var}_{x \sim P_{\lambda}} \left[ f_i (x) \right]
\end{align*}



\section{Dataset temperature}

We can define the inverse temperature as 

\begin{align*}
\frac{1}{T} &= \frac{\partial \text{H} (P_{\lambda})}{\partial U^{\lambda} (P_{\lambda})} 
= \frac{ \sum_{i=1}^{d} \frac{\partial \text{H} (P_{\lambda}) }{\partial \lambda_{i} }}{ \sum_{i=1}^{d} \frac{\partial U^{\lambda} (P_{\lambda}) }{\partial \lambda_{i} }} = \frac{ \sum_{i=1}^{d} \left( \alpha_{i} - \mathbb{E}_{x \sim P_{\lambda}} [f_{i} (x)] \right)}{ \sum_{i=1}^{d} \alpha_{i}}
\end{align*}

and therefore
$$ T = \frac{ \sum_{i=1}^{d} \alpha_{i}}{ \sum_{i=1}^{d} \left( \alpha_{i} - \mathbb{E}_{x \sim P_{\lambda}} [f_{i} (x)] \right)} $$


\section{The canonical ensemble}

See [@landau2013statistical] for basic derivations, and [@pathria2021statistical] for a detailed discussion. 

We're defining EBMs, but training them differently. 

The canonical ensemble is a powerful tool for making predictions about the behavior of systems in equilibrium. 
The maximum entropy principle is a generalization of the canonical ensemble to arbitrary constraints. 
It states that the probability distribution that maximizes the entropy subject to a set of constraints is the one that is most consistent with the constraints and the least biased. 
This principle has been used to derive a wide range of results in statistical mechanics, machine learning, and other fields. 

\section{Grand canonical ensemble}

With the average amount of data in various categories also changing, we can consider a different distribution where the corresponding $\lambda_i$ are considered potentials. 


\section{Pressure ensemble}

See also Jaynes [@jaynes1957information]. 



\section{Central limit theorem}

Khinchin [@khinchin1949mathematical] shows that



\subsection{Entropy concentration theorem}

What are the large deviations in entropy away from the maximum entropy distribution?

\subsection{Hoeffding's formula for the density}




\section{Dependence on external information}

Start with an external parameter $\gamma$ such that $\frac{\partial \lambda_i }{\partial \gamma} = 0$, 
and define $g_i^{\gamma} (x) = \frac{\partial [ f_i (x)]}{\partial \gamma}$. 
Then 

\begin{align*}
\frac{\partial \ln Z (\lambda)}{\partial \gamma} 
&= \frac{1}{Z} \frac{\partial Z (\lambda)}{\partial \gamma} 
= \frac{1}{Z} \mathbb{E} \left[ \left( \sum_{i=1}^{d} \frac{\partial [\lambda_i f_i (x)]}{\partial \gamma} \right) \exp \left( \sum_{i=1}^{d} \lambda_i f_i (x) \right) \right] \\
&= \sum_{i=1}^{d} \mathbb{E}_{x \sim P_{\lambda}} \left[ \frac{\partial [\lambda_i f_i (x)]}{\partial \gamma} \right]
= \sum_{i=1}^{d} \mathbb{E}_{x \sim P_{\lambda}} \left[ \lambda_i \frac{\partial [ f_i (x)]}{\partial \gamma} + \frac{\partial \lambda_i }{\partial \gamma} f_i (x) \right] \\
&= \sum_{i=1}^{d} \lambda_i \mathbb{E}_{x \sim P_{\lambda}} \left[ g_i^{\gamma} (x) \right]
\end{align*}

\begin{align*}
\frac{\partial \mathbb{E}_{x \sim P_{\lambda}} \left[ g_i^{\gamma} (x) \right]}{\partial \lambda_{j}}
= \frac{\partial \mathbb{E}_{x \sim P_{\lambda}} \left[ g_j^{\gamma} (x) \right]}{\partial \lambda_{i}} 
= \mathbb{E}_{x \sim P_{\lambda}} \left[ g_i^{\gamma} (x) g_j (x) \right] - \mathbb{E}_{x \sim P_{\lambda}} \left[ g_i^{\gamma} (x) \right] \mathbb{E}_{x \sim P_{\lambda}} \left[ g_j^{\gamma} (x) \right]
\end{align*}

% - Differential relations from https://en.wikipedia.org/wiki/Helmholtz_free_energy#Relating_free_energy_to_other_variables



\section{Jarzynski equality and Crooks fluctuations}

\begin{align*}
\mathbb{E}_{x \sim P_{\lambda}} \left[ \exp \left( U^{\lambda} (x) \right) \right] = 1
\end{align*}

For any antisymmetric feature $\omega$, we can show a similar equality. 

\begin{align*}
\mathbb{E}_{x \sim P_{\lambda}} \left[ \exp \left( - \omega \right) \right] = 1
\end{align*}

Now let's define $\omega$ to be the entropy production in transitioning from $P_{I} \to P_{F}$:

\begin{align*}
\omega := \text{H} (x, P_{F}) - \text{H} (x, P_{I}) - \delta Q
\end{align*}

where we remember the definition of heat $\delta Q := \sum_{i=1}^{d} \lambda_{i} [\delta Q_i^{\lambda}]$, such that 
$d U^{\lambda} (P_{\lambda})
= \sum_{i=1}^{d} \left[ \lambda_{i} [\delta Q_i^{\lambda}] + \mathbb{E}_{x \sim P_{\lambda}} \left[ d U_i^{\lambda} (x) \right] \right]$

where the ``heat change" associated with a given feature $i$ is 
$$ \delta Q_i^{\lambda} := \mathbb{E}_{x \sim P_{\lambda}} \left[ \Delta_{i} (x) \right] - \Delta_{i}^{\alpha} $$

Now $P_{i} (x) := \exp \left( F^{\lambda_{i}} (P_{\lambda_{i}}) - U^{\lambda_{i}} (x) \right)$, so 

\begin{align*}
\omega &= - F^{\lambda_{F}} (P_{\lambda_{F}}) + U^{\lambda_{F}} (P_{\lambda_{F}}) + F^{\lambda_{I}} (P_{\lambda_{I}}) - U^{\lambda_{i}} (P_{\lambda_{I}}) + \delta Q \\
&= - \Delta F^{\lambda} (P_{\lambda}) + \Delta U^{\lambda} (P_{\lambda}) - \delta Q
= - \Delta F^{\lambda} (P_{\lambda}) + \mathbb{E}_{x \sim P_{\lambda}} \left[ \Delta U^{\lambda} (x) \right]
\end{align*}

This quantifies entropy production in a process of any kind, even far from equilibrium (i.e. without adjusting $\lambda$) \cite{crooks1999entropy}. 

It implies that $\mathbb{E}_{x \sim P_{\lambda}} \left[ \exp \left( - \omega \right) \right] = 1$, i.e. $\omega \geq 0$, so 

$$\Delta F^{\lambda} (P_{\lambda}) \leq \mathbb{E}_{x \sim P_{\lambda}} \left[ \Delta U^{\lambda} (x) \right]$$


\section{Fluctuation-dissipation theorem}

The book \cite{pathria2021statistical} has a statement. 

The fluctuation-dissipation theorem relates the response of a system to an external perturbation to the fluctuations of the system in equilibrium.

The theorem can be stated as follows. 

Consider a system in equilibrium with a heat bath at temperature $T$. 
Let $x$ be a state variable of the system, and let $f(x)$ be a feature function of the system. 
Let $p(x)$ be the probability distribution over states of the system. 
Let $p(x + \delta x)$ be the probability distribution over states of the system when the state variable is perturbed by $\delta x$. 
Then the fluctuation-dissipation theorem states that the response of the system to the perturbation is related to the fluctuations of the system in equilibrium by the following equation: 

\begin{align*}
\mathbb{E}_{x \sim p} [f(x + \delta x) - f(x)] = - \beta \mathbb{E}_{x \sim p} [f(x)] \delta x
\end{align*}

where $\beta = 1/T$ is the inverse temperature of the heat bath.



\section{Algorithmic consequences}

Calculate entropy change with learning

Easy to fine-tune by adding a couple more features. Free energy will only decrease, right? Measure this. 



\section{Distribution shift and heat}

Any change in the data or constraints will decompose into these two (work + heat). 
The predicted distribution of the data is determined completely by the data's energy levels, so **work** - the change in those - is meaningfully easier to adapt to. 
The difficulty is in account for changes in constraints that are not accounted for by the existing data. 
This is what **heat** represents in this context -- the change in performance (internal energy) that is not due to the change in the data's energy levels (predictions). 

Note that the probability distribution could specialize over a subset of the data, in which case we can restrict to those parts of the data, and only those energies matter. 


Try this for a simple example with a logistic regressor where the data changes, and decompose the change in performance of the regressor (change in the free energy) into work and heat. 
We've shown that the score function is determined by the internal energy, and the regret is determined by the free energy. 
Take it through a zero-heat process, all adiabatic, where the regret doesn't change because the energy is conserved. 



the book [@thompson2015mathematical] contains more examples.



